A Finite Element Discretization of the Streamfunction Formulation of the Stationary Quasi-Geostrophic Equations of the Ocean

This paper presents a conforming finite element discretization of the streamfunction formulation of the one-layer stationary quasi-geostrophic equations, which are a commonly used model for the large scale wind- driven ocean circulation. Optimal error estimates for this finite element discretization with the Argyris element are derived. Numerical tests for the finite element discretization of the quasi-geostrophic equations and two of its standard simplifications (the linear Stommel model and the linear Stommel-Munk model) are carried out. By benchmarking the numerical results against those in the published literature, we conclude that our finite element discretization is accurate. Furthermore, the numerical results have the same convergence rates as those predicted by the theoretical error estimates.

==> Argyris.Triangle.tex <==
\begin{figure}
	\begin{center}
\begin{tikzpicture}[scale=0.5]
	%define the vertices of the triangle
	\path[coordinate] (0,0) coordinate(A)
		++(60:3cm) coordinate(D)
		++(60:3cm) coordinate(B)
		++(-60:3cm) coordinate(E)
		++(-60:3cm) coordinate(C)
		++(180:3cm) coordinate(F);
	%label the vertices and draw edges
	\draw (A) -- (D) -- (B) -- (E) -- (C) -- (F) -- cycle;
	%draw the interpolation points
	%function values
	\filldraw[black] (A) circle(3pt); 
	\filldraw[black] (B) circle(3pt); 
	\filldraw[black] (C) circle(3pt); 
	%first derivatives
	\draw[black] (A) circle(6pt); 
	\draw[black] (B) circle(6pt); 
	\draw[black] (C) circle(6pt); 
	%second derivatives
	\draw[black] (A) circle(9pt); 
	\draw[black] (B) circle(9pt); 
	\draw[black] (C) circle(9pt); 
	%normal derivatives
	\draw (1.067,2.848) -- (D) -- (1.933,2.348); 
	\draw (4.067,2.348) -- (E) -- (4.933,2.848); 
	\draw (3,-0.5cm) -- (F) -- (3,0.5cm); 
	%labels
%	\node[below of=A, node distance=0.5cm] (k) {$k=j+1$};
% \node[above of=B, node distance=0.5cm] (j) {$j=i+1$};
%	\node[below of=C, node distance=0.5cm] (i) {$i$};
\end{tikzpicture}
	\end{center}
	\caption{Argyris element with its 21 degrees of freedom.}
	\label{fig:Argyris}
\end{figure}


==> Argyris.tex <==
  If we are to require conforming finite elements, Lagrange finite elements are not enough to
  guarantee continuity in the first derivative, and so to ensure continuity in the first derivative
  \cite{Johnson} the Argyris Element (depicted in \autoref{fig:Argyris}) was implemented in our
  numerical tests. The Argyris element is probably the best known of all $C^1$ finite elements
  \cite{Argyris,Dominguez06}, but appear to be rarely implemented. 

  \input{Argyris.Triangle.tex}

  The Argyris element ensures $C^1$ continuity \cite{Ciarlet,Dominguez06,Okabe}, but at a cost
  of twenty-one degrees of freedom.  These twenty-one degrees of freedom, however, give basis
  polynomials of degree five. 
  Thus, the Argyris element has a high rate of convergence \cite{Ciarlet,Dominguez06}.
  The degrees of freedom include the value at each vertex, the value of the first derivatives at
  each vertex, the value of the second derivatives at each vertex, the value of the mixed derivative
  at each vertex, and finally the value of the normal derivatives at each of the edge midpoints.
  Herein lies the main difficulty in implementing the Argyris element, the normal derivatives. Not
  only do we now have twenty-one degrees of freedom that we must worry about, but the added complexity of a
  transformation that maintains the direction of the normal derivations is also required. Since working
  on the reference element is the most common way of working finite elements and normal derivatives
  are not preserved by affine transformations, a more complicated transformation has to be
  employed. This is unlike a standard Lagrange finite element, where only a simple affine transformation is
  required \cite{Dominguez06}.

  Dominguez \emph{et al.} \cite{Dominguez06} developed such a transformation. This transformation, which is a $21
  \times 21$ matrix, allows for all calculations to be done on a reference element, vastly
  simplifying the calculations for the various matrices and load vector required for the QGE FE calculations and allowing for faster running code. 
We emphasize that special care needs to be taken to ensure that the normal derivatives point in the same direction across triangles.


==> Error.tex <==
The main goal of this section is to develop a rigorous numerical analysis for the FE discretization of the QGE \eqref{eqn:FEForm} by using the conforming Argyris element.
First, in Theorem~\ref{thm:EnergyNorm} we prove error estimates in the $H^2$ norm by using an approach similar to that used in \cite{Cayco86}.
Second, in Theorem~\ref{thm:Errors}, we prove error estimates in the $L^2$ and $H^1$ norms by using a duality argument.

\begin{theorem}
\label{thm:EnergyNorm}
  Let $\psi$ be the solution of \eqref{eqn:WeakForm} and $\psi^h$ be the solution
  of \eqref{eqn:FEForm}. 
  Furthermore, assume that the following small data condition is satisfied:
  \begin{eqnarray}
  Re^{-2} \, Ro 
  \geq \Gamma_1 \, \| F \|_{-2} ,
  \label{eqn:small_data_condition}
  \end{eqnarray}
where 
$Re$ is the Reynolds number defined in \eqref{eqn:reynolds_number}, 
$Ro$  is the Rossby number defined in \eqref{eqn:rossby_number},
 $\Gamma_1$ is the continuity constant of the trilinear form $a_1$ in \eqref{eqn:a1cont}, and 
 $F$ is the forcing term.
Then the following error estimate holds:
  \begin{equation}
    |\psi - \psi^h|_2 
    \le C(Re, Ro, \Gamma_1, \Gamma_2, F) \, \inf_{\chi^h \in X^h} |\psi - \chi^h|_2 ,
    \label{eqn:EnergyNorm}
  \end{equation}
  where $\Gamma_2$ is the continuity constant of the bilinear form $a_2$ in \eqref{eqn:a2Cont} and 
  \begin{eqnarray} 
  C(Re, Ro, \Gamma_1, F)
  := %\left[
  \frac{
   Ro^{-1} \, \Gamma_2
  + 2 \, Re^{-1} 
  + \Gamma_1 \, Re \, Ro^{-1} \, \| F \|_{-2}
  }
  {
  Re^{-1}
  - \Gamma_1 \, Re \, Ro^{-1} \, \| F \|_{-2}
  }
  %\right]
  \label{eqn:constant_definition}
  \end{eqnarray}
is a generic constant that can depend on $Re$, $Ro$, $\Gamma_1$, $\Gamma_2$, $F$, but {\it not} on the meshsize $h$.
\end{theorem}

\begin{remark}
Note that the small data condition in Theorem~\ref{thm:EnergyNorm} involves {\it both} the Reynolds number and the Rossby number, the latter quantifying the rotation effects in the QGE.

Furthermore, note that the standard small data condition $Re^{-2} \geq \Gamma_1 \, \| F \|_{-2}$ used to prove the uniqueness for the steady-state 2D NSE \cite{Girault79,Girault86,layton2008introduction,temam2001navier} is significantly more restrictive for the QGE, since \eqref{eqn:small_data_condition} has the Rossby number (which is small when rotation effects are significant) on the left-hand side.
This is somewhat counterintuitive, since in general rotation effects are expected to help in proving the well-posedness of the system.
We think that the explanation for this puzzling situation is the following: 
Rotation effects do make the mathematical analysis of 3D flows more amenable by giving them a 2D character.
We, however, are concerned with 2D flows (the QGE).
In this case, the small data condition \eqref{eqn:small_data_condition} (needed in proving the uniqueness of the solution) indicates that rotation effects make the mathematical analysis of the (2D) QGE more complicated than that of the 2D NSE.
%We emphasize that there is no contradiction, since, although the rotation effects do help in the three-dimensional case, they seem to complicate the situation if one compare the QGE with the two-dimensional (not the three-dimensional) NSE.
\end{remark}
\begin{proof}
  Since $X^h \subset X$, \eqref{eqn:WeakForm} holds for all $\chi = \chi^h\in X^h$.
  Subtracting \eqref{eqn:FEForm} from \eqref{eqn:WeakForm} with $\chi=\chi^h \in
  X^h$ gives
  \begin{equation}
    \begin{split}
      a_0(\psi - \psi^h,\chi^h) + a_1(\psi,\psi,\chi^h) -
      a_1(\psi^h,\psi^h,\chi^h) \\ 
      + a_2(\psi-\psi^h,\chi^h) = 0 \qquad \forall \chi^h \in
    X^h.
  \end{split}
    \label{eqn:ErrorEq}
  \end{equation}
  Next, adding and subtracting $a_1(\psi^h,\psi,\chi^h)$ to \eqref{eqn:ErrorEq}, we get:
  \begin{eqnarray}
    %\begin{split}
      && a_0(\psi - \psi^h,\chi^h) + a_1(\psi,\psi,\chi^h) - a_1(\psi^h,\psi,\chi^h) %\\
      + a_1(\psi^h,\psi,\chi^h) - a_1(\psi^h,\psi^h,\chi^h) \nonumber \\
      && \hspace*{3.0cm} + a_2(\psi-\psi^h,\chi^h) = 0 \qquad \forall \chi^h \in X^h.
    %\end{split}
    \label{eqn:interError}
  \end{eqnarray}
  The error $e$ can be decomposed as 
  \begin{equation}
    e:= \psi-\psi^h = (\psi-\lambda^h)+(\lambda^h-\psi^h):= \eta + \varphi^h,
    \label{eqn:ErrorTrick}
  \end{equation}
  where $\lambda^h\in X^h$ is arbitrary. 
  Thus, equation \eqref{eqn:interError} can be
  rewritten as 
  \begin{equation}
    \begin{split}
      a_0(\eta+\varphi^h,\chi^h)+a_1(\eta+\varphi^h,\psi,\chi^h)+a_1(\psi^h,\eta+\varphi^h,\chi^h) \\
      + a_2(\eta+\varphi^h,\chi^h)=0 \qquad \forall \chi^h \in X^h.
    \end{split}
    \label{eqn:ErrorEta}
  \end{equation}
  Letting $\chi^h := \varphi^h$ in \eqref{eqn:ErrorEta}, we obtain 
  \begin{equation}
    \begin{split}
      a_0(\varphi^h,\varphi^h) + a_2(\varphi^h,\varphi^h) = -a_0(\eta,\varphi^h)
      - a_1(\eta,\psi,\varphi^h) - a_1(\varphi^h,\psi,\varphi^h) \\
      - a_1(\psi^h,\eta,\varphi^h) - a_1(\psi^h,\varphi^h,\varphi^h)
      -a_2(\eta,\varphi^h).
    \end{split}
    \label{eqn:ErrorVarphi}
  \end{equation}
  Note that, since $a_2(\varphi^h,\varphi^h)=-a_2(\varphi^h,\varphi^h)\; \forall
  \varphi^h \in X^h \subset X = H^2_0$ (see \eqref{eqn:stability_4} in the proof of Theorem \ref{thm:stability}), it follows that 
  \begin{equation}
    a_2(\varphi^h,\varphi^h)=0 .
    \label{eqn:a20}
  \end{equation}
  Also, it follows immediately from \eqref{eqn:a1} that
  \begin{equation}
    a_1(\psi^h,\varphi^h,\varphi^h)=0 .
    \label{eqn:a10}
  \end{equation}
  Combining \eqref{eqn:ErrorVarphi}, \eqref{eqn:a20}, and \eqref{eqn:a10}, we get:
  \begin{equation}
    \begin{split}
      a_0(\varphi^h,\varphi^h) = -a_0(\eta,\varphi^h)
      - a_1(\eta,\psi,\varphi^h) - a_1(\varphi^h,\psi,\varphi^h) \\
      - a_1(\psi^h,\eta,\varphi^h) - a_2(\eta,\varphi^h).
    \end{split}
    \label{eqn:ErrorZeroed}
  \end{equation}
  Using
  \begin{equation*}
    a_0(\varphi^h,\varphi^h) = Re^{-1} \, |\varphi^h|^2_2
  \end{equation*}
  and inequalities \eqref{eqn:a0} -- \eqref{eqn:a2} in equation
  \eqref{eqn:ErrorZeroed} gives
  \begin{equation}
    \begin{split}
      Re^{-1} \, |\varphi^h|^2_2 \le Re^{-1} \,  |\eta|_2 \, |\varphi^h|_2 + \Gamma_1
      \biggl( |\eta|_2 \, |\psi|_2 \, |\varphi^h|_2 + |\psi^h|_2 \, |\eta|_2 \, |\varphi^h|_2 \biggr) \\ 
      + \Gamma_1 \, |\varphi^h|^2_2 \, |\psi|_2 + Ro^{-1} \, \Gamma_2 \, |\eta|_2 \, |\varphi^h|_2 .
    \end{split}
    \label{eqn:varphiIneq}
  \end{equation}
  Simplifying and rearranging terms in \eqref{eqn:varphiIneq} gives
  \begin{equation}
      |\varphi^h|_2 
      \le 
      \left(
      Re^{-1}
      - \Gamma_1 \, | \psi |_2
      \right)^{-1} \, 
      \left(
      Re^{-1} 
      + \Gamma_1 \, |\psi|_2 
      + \Gamma_1 \, |\psi^h|_2 
      + Ro^{-1} \, \Gamma_2
      \right) \,  
      |\eta|_2 .
    \label{eqn:phihIneq}
  \end{equation}
  Using \eqref{eqn:phihIneq} and the triangle inequality along with the stability estimates \eqref{eqn:stability_1} and \eqref{eqn:stability_fem_1} gives
  \begin{align}
    |e|_2 
    &\le |\eta|_2 
    + |\varphi^h|_2 \nonumber \\[0.2cm]
    &\le \left[
    1 
    + \frac{Re^{-1} 
      + \Gamma_1 \, |\psi|_2 
      + \Gamma_1 \, |\psi^h|_2 
      + Ro^{-1} \, \Gamma_2} {Re^{-1} 
      - \Gamma_1 \, |\psi|_2} 
      \right] \, |\eta|_2 \nonumber \\[0.2cm]
    &\le \left[
    1 
    + \frac{Re^{-1} 
      + \Gamma_1 \, \left( Re \, Ro^{-1} \, \| F \|_{-2} \right) 
      + \Gamma_1 \, \left( Re \, Ro^{-1} \, \| F \|_{-2} \right) 
      + Ro^{-1} \, \Gamma_2} {Re^{-1} 
      - \Gamma_1 \, \left( Re \, Ro^{-1} \, \| F \|_{-2} \right) } 
      \right] \, |\eta|_2 \nonumber \\
  &= 
  \left[
  \frac{
  Ro^{-1} \, \Gamma_2
  + 2 \, Re^{-1} 
  + \Gamma_1 \, Re \, Ro^{-1} \, \| F \|_{-2}
  }
  {
  Re^{-1}
  - \Gamma_1 \, Re \, Ro^{-1} \, \| F \|_{-2}
  }
  \right] \, | \psi-\lambda^h |_2 ,
    \label{eqn:EnergyError}
  \end{align}
where $\lambda^h \in X^h$ is arbitrary.
Taking the infimum over $\lambda^h \in X^h$ in \eqref{eqn:EnergyError} proves the error estimate \eqref{eqn:EnergyNorm}.
\hfill 
\end{proof}

In Theorem~\ref{thm:EnergyNorm}, we proved an error estimate in the $H^2$ seminorm.
In Theorem~\ref{thm:Errors}, we will prove error estimates in the $L^2$ norm and $H^1$ seminorm by using a duality argument.
To this end, we first notice that the QGE \eqref{qge_psi_3} can be written as
\begin{eqnarray}
\mathcal{N} \, \psi
= Ro^{-1} \, F ,
\label{eqn:qge_operator_formulation}
\end{eqnarray}
where the nonlinear operator $\mathcal{N}$ is defined as
\begin{eqnarray}
\mathcal{N} \, \psi
:= Re^{-1} \, \Delta^2 \psi 
+ J(\psi , \Delta \psi)
- Ro^{-1} \, \frac{\partial \psi}{\partial x} .
\label{eqn:nonlinear_operator}
\end{eqnarray}
The linearization of $\mathcal{N}$ around $\psi$, a solution of \eqref{qge_psi_3}, yields the following {\it linear} operator:
\begin{eqnarray}
\mathcal{L} \, \chi
:= Re^{-1} \, \Delta^2 \chi 
+ J(\chi , \Delta \psi)
+ J(\psi, \Delta \chi)
- Ro^{-1} \, \frac{\partial \chi}{\partial x} .
\label{eqn:linear_operator}
\end{eqnarray}
To find the dual problem associated with the QGE \eqref{eqn:qge_operator_formulation}, we first define the {\it dual operator} $\mathcal{L}^*$ of $\mathcal{L}$:
\begin{eqnarray}
(\mathcal{L} \, \chi , \psi^*)
= ( \chi , \mathcal{L}^* \, \psi^*)
\qquad 
\forall \, \psi^* \in X .
\label{eqn:dual_operator}
\end{eqnarray}
To find $\mathcal{L}^*$, we use the standard procedure: 
In \eqref{eqn:dual_operator}, we use the definition of $\mathcal{L}$ given in \eqref{eqn:linear_operator} and we ``integrate by parts" (i.e., we use Green's theorem):
\begin{eqnarray}
\hspace*{-0.4cm}
(\mathcal{L} \, \chi , \psi^*)
&=& \left( 
Re^{-1} \, \Delta^2 \chi 
+ J(\chi , \Delta \psi)
+ J(\psi, \Delta \chi)
- Ro^{-1} \, \frac{\partial \chi}{\partial x} 
\, , \, \psi^*
\right) 
\nonumber \\
&=& \left( 
\chi \, , \, 
Re^{-1} \, \Delta^2 \, \psi^*
- J(\psi , \Delta \psi^* )
+ Ro^{-1} \, \frac{\partial \psi^*}{\partial x} 
\right)
+ \biggl( J(\chi , \Delta \psi) , \psi^* \biggr) ,
\label{eqn:dual_operator_1}
\end{eqnarray}
where to get the first term on the right-hand side of \eqref{eqn:dual_operator_1} we used the skew-symmetry of the trilinear form $a_1$ in the last two variables and Green's theorem (just as we did in the proof of Theorem \ref{thm:stability}).
Next, we apply Green's theorem to the second term on the right-hand side of \eqref{eqn:dual_operator_1}:
\begin{eqnarray}
\biggl( J(\chi , \Delta \psi) , \psi^* \biggr)
&=& \chi_x \, \Delta \psi_y \, \psi^*
   -    \chi_y \, \Delta \psi_x \, \psi^*
\nonumber \\
&\stackrel{Green}{=}& 
- \chi \, \Delta \psi_{y x} \, \psi^* 
- \chi \, \Delta \psi_y \, \psi^*_x
+ \chi \, \Delta \psi_{x y} \, \psi^* 
+ \chi \, \Delta \psi_x \, \psi^*_y
\nonumber \\
&=& \biggl( \chi , J(\Delta \psi , \psi^*) \biggr) .
\label{eqn:dual_operator_2}
\end{eqnarray}
Equations \eqref{eqn:dual_operator_1}-\eqref{eqn:dual_operator_2} imply:
\begin{eqnarray}
(\mathcal{L} \, \chi , \psi^*)
&=& \left( 
\chi \, , \, 
Re^{-1} \, \Delta^2 \, \psi^*
- J(\psi , \Delta \psi^* )
+ Ro^{-1} \, \frac{\partial \psi^*}{\partial x} 
\right)
+ \biggl( \chi , J(\Delta \psi , \psi^*) \biggr)
\nonumber \\
&=& ( \chi , \mathcal{L}^* \, \psi^*) .
\label{eqn:dual_operator_3}
\end{eqnarray}
Thus, the {\it dual operator} $\mathcal{L}^*$ is given by
\begin{eqnarray}
\mathcal{L}^* \, \psi^*
= Re^{-1} \, \Delta^2 \, \psi^*
- J(\psi , \Delta \psi^* )
+ J(\Delta \psi , \psi^* )
+ Ro^{-1} \, \frac{\partial \psi^*}{\partial x} .
\label{eqn:dual_operator_4}
\end{eqnarray}
For any given $g \in L^2(\Omega)$, the weak formulation of the {\it dual problem} is:
\begin{eqnarray}
( \mathcal{L}^* \, \psi^* , \chi )
= (g , \chi)
\qquad
\forall \, \chi \in X = H_0^2(\Omega) .
\label{eqn:dual_operator_5}
\end{eqnarray}
We assume that $\psi^*$, the solution of \eqref{eqn:dual_operator_5}, satisfies the following elliptic regularity estimates:
\begin{eqnarray}
&& \psi^* \in H^4(\Omega) \cap H^2_0(\Omega), 
\label{eqn:dual_operator_6a} \\[0.2cm]
&& \| \psi^* \|_4 
\le C \, \|g\|_{0},
\label{eqn:dual_operator_6b} \\[0.2cm]
&& \| \psi^* \|_3 
\le C \, \|g\|_{-1},
\label{eqn:dual_operator_6c}
\end{eqnarray}
where $C$ is a generic constant that can depend on the data, but not on the meshsize $h$.
\begin{remark}
We note that this type of elliptic regularity was also assumed in \cite{Cayco86} for the streamfunction formulation of the 2D NSE.
In that report, it was also noted that, for a polygonal domain with maximum interior vertex angle $\theta < 126^{\circ}$, the assumed elliptic regularity was actually proved by Blum and Rannacher \cite{blum1980boundary}.
We note that the theory developed in \cite{blum1980boundary} carries over to our case as well.
In Section 5 in \cite{blum1980boundary} it is proved that, for weakly nonlinear problems that involve the biharmonic operator as linear main part and that satisfy certain growth restrictions, each weak solution satisfies elliptic regularity results of the form \eqref{eqn:dual_operator_6a}-\eqref{eqn:dual_operator_6c}.
Assuming that $\Omega$ is a bounded polygonal domain with inner angle $\omega$ at each boundary corner satisfying $\omega < 126.283696\ldots^{\circ}$, Theorem 7 in \cite{blum1980boundary} with $k = 0$ and $k = 1$ implies \eqref{eqn:dual_operator_6a}-\eqref{eqn:dual_operator_6c}.
Using an argument similar to that used in Section 6(b) in \cite{blum1980boundary} to prove that the streamfunction formulation of the 2D NSE satisfies the restrictions in Theorem 7, we can prove that $\psi^*$, the solution of our dual problem \eqref{eqn:dual_operator_5}, satisfies the elliptic regularity results in \eqref{eqn:dual_operator_6a}-\eqref{eqn:dual_operator_6c}.
Indeed, the main point in Section 6(b) in \cite{blum1980boundary} is that the corner singularities arising in flows around sharp corners are essentially determined by the linear main part $\Delta^2$ in the streamfunction formulation of the 2D NSE, which is the linear main part of our dual problem \eqref{eqn:dual_operator_5} as well.
\end{remark}

The error estimates in the $L^2$ norm and $H^1$ seminorm that we prove in Theorem~\ref{thm:Errors} are
derived for the particular space $X^h\subset H^2_0(\Omega)$ consisting of Argyris elements, although
the same results can be derived for other conforming $C^1$ FE spaces. 
\begin{theorem} \label{thm:Errors}
  Let $\psi$ be the solution of \eqref{eqn:WeakForm} and $\psi^h$ be the solution
  of \eqref{eqn:FEForm}. 
  Assume that the same small data condition as in Theorem \ref{thm:EnergyNorm} is satisfied:
  \begin{eqnarray}
  Re^{-2} \, Ro 
  \geq \Gamma_1 \, \| F \|_{-2} .
  \label{eqn:small_data_condition_dual}
  \end{eqnarray}
  Furthermore, assume that $\psi\in H^6(\Omega) \cap H^2_0(\Omega)$. 
  Then there exist positive constants $C_0, \, C_1 \text{ and } C_2$ that can depend on $Re$, $Ro$, $\Gamma_1$, $\Gamma_2$, $F$, but {\it not} on the meshsize $h$, such that
  \begin{align}
    |\psi - \psi^h|_2 &\le C_2 \, h^4 , \label{eqn:H2Error} \\
    |\psi - \psi^h|_1 &\le C_1 \, h^5 , \label{eqn:H1Error} \\
    \|\psi - \psi^h\|_0 &\le C_0 \, h^6 . \label{eqn:L2Error}
  \end{align}
\end{theorem}
\begin{proof}
Estimate \eqref{eqn:H2Error} follows immediately from \eqref{eqn:argyris_approximation_0} and Theorem \ref{thm:EnergyNorm}. 
Estimates \eqref{eqn:L2Error} and \eqref{eqn:H1Error} follow from a duality argument.

The error in the primal problem \eqref{eqn:WeakForm} and the interpolation error in the dual problem  \eqref{eqn:dual_operator_5} (with the function $g$ to be specified later) are denoted as
\begin{eqnarray}
e
:= \psi
- \psi^h 
\qquad
e^*
: = \psi^*
- {\psi^*}^h ,
\label{eqn:theorem_dual_1}
\end{eqnarray}
respectively.

We start proving the $L^2$ norm estimate \eqref{eqn:L2Error}.
For this case, the function that we consider in the dual problem \eqref{eqn:dual_operator_5} has the form $g = e$.
\begin{eqnarray}
|e|^2
= (e , e)
&=& (\mathcal{L} \, e , \psi^*)
= (e , \mathcal{L}^* \, \psi^*)
\nonumber \\
&=& (e , \mathcal{L}^* \, e^*)
+ (e , \mathcal{L}^* \, {\psi^*}^h)
= (\mathcal{L} \, e , e^*)
+ (\mathcal{L} \, e , {\psi^*}^h) .
\label{eqn:theorem_dual_2}
\end{eqnarray}
The last term on the right-hand side of \eqref{eqn:theorem_dual_2} is given by
\begin{eqnarray}
(\mathcal{L} \, e , {\psi^*}^h)
= \left(
Re^{-1} \, \Delta^2 e
+ J(e , \Delta \, \psi)
+ J(\psi , \Delta \, e)
- Ro^{-1} \, \frac{\partial e}{\partial x}
 \, , \,  
{\psi^*}^h
\right) .
\label{eqn:theorem_dual_3}
\end{eqnarray}
To estimate this term, we consider the error equation obtained by subtracting \eqref{eqn:FEForm} (with $\psi^h= {\psi^*}^h$) from \eqref{eqn:WeakForm} (with $\chi = {\psi^*}^h$):
\begin{eqnarray}
\left(
Re^{-1} \, \Delta^2 e
- Ro^{-1} \, \frac{\partial e}{\partial x}
 \, , \,  
{\psi^*}^h
\right)
+ \left(
J(\psi , \Delta \, \psi)
- J(\psi^h , \Delta \, \psi^h)
 \, , \,  
{\psi^*}^h
\right)
= 0 .
\label{eqn:theorem_dual_4}
\end{eqnarray}
Using \eqref{eqn:theorem_dual_4}, equation \eqref{eqn:theorem_dual_3} can be written as follows:
\begin{eqnarray}
(\mathcal{L} \, e , {\psi^*}^h)
= \left(
J(e , \Delta \, \psi)
+ J(\psi , \Delta \, e)
- J(\psi , \Delta \, \psi)
+ J(\psi^h , \Delta \, \psi^h)
 \, , \,  
{\psi^*}^h
\right) .
\label{eqn:theorem_dual_5}
\end{eqnarray}
Thus, by using \eqref{eqn:theorem_dual_5} equation \eqref{eqn:theorem_dual_2} becomes:
\begin{eqnarray}
|e|^2
&=& (\mathcal{L} \, e , e^*)
+ (\mathcal{L} \, e , {\psi^*}^h)
\nonumber \\
&=& Re^{-1} \, (\Delta e , \Delta e^*)
- Ro^{-1} \, \left( \frac{\partial e}{\partial x} , e^* \right)
+ \left(
J(e , \Delta \psi)
+ J(\psi , \Delta e)
, e^*
\right)
\nonumber \\
&+& \left(
  J(e , \Delta \, \psi)
+ J(\psi , \Delta \, e)
- J(\psi , \Delta \, \psi)
+ J(\psi^h , \Delta \, \psi^h)
 \, , \,  
{\psi^*}^h
\right) 
\nonumber \\
&=& a_0(e , e^*)
+ a_2(e , e^*)
+ a_1(e , \psi , e^*)
+ a_1(\psi , e, e^*)
+ a_1(e , \psi , {\psi^*}^h)
\nonumber \\
&& + a_1(\psi , e , {\psi^*}^h)
- a_1(\psi , \psi , {\psi^*}^h)
+ a_1(\psi^h , \psi^h , {\psi^*}^h)
\nonumber \\
&=& a_0(e , e^*)
+ a_2(e , e^*)
+ a_1(e , \psi , e^*)
+ a_1(\psi , e, e^*)
\nonumber \\
&& - a_1(e , \psi , e^*)
+ a_1(e , \psi^h , e^*)
+ a_1(e , e , \psi^*)
\label{eqn:theorem_dual_6}
\end{eqnarray}
Using the bounds in \eqref{eqn:a0Cont}-\eqref{eqn:a2Cont}, \eqref{eqn:theorem_dual_6} yields:
\begin{eqnarray}
|e|^2
&=& a_0(e , e^*)
+ a_2(e , e^*)
+ a_1(e , \psi , e^*)
+ a_1(\psi , e, e^*)
\nonumber \\
&& - a_1(e , \psi , e^*)
+ a_1(e , \psi^h , e^*)
+ a_1(e , e , \psi^*)
\nonumber \\
&\leq& Re^{-1} \, | e |_2 \, |e^* |_2
+ Ro^{-1} \, \Gamma_2 \, | e |_2 \, |e^* |_2
+ \Gamma_1 \, | e |_2 \, | \psi |_2 \, | e^* |_2
+ \Gamma_1 \, | \psi |_2 \, | e |_2 \, | e^* |_2
\nonumber \\
&& + \Gamma_1 \, | e |_2 \, | \psi |_2 \, | e^* |_2
+ \Gamma_1 \, | e |_2 \, | \psi^h |_2 \, | e^* |_2
+ \Gamma_1 \, | e |_2 \, | e |_2 \, | \psi^* |_2
\nonumber \\
&=& | e |_2 \, |e^* |_2 \, 
\left(
Re^{-1}
+ Ro^{-1} \, \Gamma_2
+ \Gamma_1 \, | \psi |_2 
+ \Gamma_1 \, | \psi |_2
+ \Gamma_1 \, | \psi |_2
+ \Gamma_1 \, | \psi^h |_2
\right)
\nonumber \\
&& + | e |_2^2 \, 
\left(
\Gamma_1 \, | \psi^* |_2
\right) .
\label{eqn:theorem_dual_7}
\end{eqnarray}
We start bounding the terms on the right-hand side of \eqref{eqn:theorem_dual_7}.
First, we note that using the stability estimates \eqref{eqn:stability_1} for $\psi$ and \eqref{eqn:stability_fem_1} for $\psi^h$, the right-hand side of \eqref{eqn:theorem_dual_7} can be bounded as follows:
\begin{eqnarray}
|e|^2
\leq C \, | e |_2 \, |e^* |_2
+ | e |_2^2 \, 
\left(
\Gamma_1 \, | \psi^* |_2
\right) ,
\label{eqn:theorem_dual_8}
\end{eqnarray}
where $C$ is a generic constant that can depend on $Re$, $Ro$, $\Gamma_1$, $\Gamma_2$, $F$, but {\it not} on the meshsize $h$.
By using the approximation results \eqref{eqn:argyris_approximation_1}, we get:
\begin{eqnarray}
|e^* |_2
\leq C \, h^2 \, | \psi^* |_4 .
\label{eqn:theorem_dual_9}
\end{eqnarray}
By using \eqref{eqn:dual_operator_6a} and \eqref{eqn:dual_operator_6b}, the elliptic regularity results of the dual problem \eqref{eqn:dual_operator_5} with $g := e$, we also get:
\begin{eqnarray}
| \psi^* |_4
\leq C \, | e | ,
\label{eqn:theorem_dual_10}
\end{eqnarray}
which obviously implies
\begin{eqnarray}
| \psi^* |_2
\leq C \, | e | .
\label{eqn:theorem_dual_11}
\end{eqnarray}
Inequalities \eqref{eqn:theorem_dual_9}-\eqref{eqn:theorem_dual_10} imply:
\begin{eqnarray}
|e^* |_2
\leq C \, h^2 \, | e | .
\label{eqn:theorem_dual_12}
\end{eqnarray}
Inserting \eqref{eqn:theorem_dual_11} and \eqref{eqn:theorem_dual_12}  in \eqref{eqn:theorem_dual_8}, we get:
\begin{eqnarray}
|e|^2
\leq C \, h^2 \, | e |_2 \, | e |
+ C \, | e |_2^2 \, | e | .
\label{eqn:theorem_dual_13}
\end{eqnarray}
Using the obvious simplifications and the $H^2$ error estimate \eqref{eqn:H2Error} in \eqref{eqn:theorem_dual_13} yields:
\begin{eqnarray}
|e|
\leq C \, h^2 \, | e |_2
+ C \, | e |_2^2
\leq C \, h^6 + C \, h^8
= C_0 \, h^6 ,
\label{eqn:theorem_dual_14}
\end{eqnarray}
which proves the $L^2$ error estimate \eqref{eqn:L2Error}.

Next, we prove the $H^1$ seminorm estimate \eqref{eqn:H1Error}.
Since the duality approach we use is similar to that we used in proving the  $L^2$ norm estimate \eqref{eqn:L2Error}, we only highlight the main differences.
For this case, the function that we consider in the dual problem \eqref{eqn:dual_operator_5} has the form $g = - \Delta e$.
We start again by writing the $H^1$ norm of the error in terms of the dual operator $\mathcal{L}^*$:
\begin{eqnarray}
|e|_1^2
&=& (\nabla e , \nabla e)
= ( e , - \Delta e)
= (\mathcal{L} \, e , \psi^*)
= (e , \mathcal{L}^* \, \psi^*)
\nonumber \\
&=& (e , \mathcal{L}^* \, e^*)
+ (e , \mathcal{L}^* \, {\psi^*}^h)
= (\mathcal{L} \, e , e^*)
+ (\mathcal{L} \, e , {\psi^*}^h) .
\label{eqn:theorem_dual_15}
\end{eqnarray}
Thus, the second and fourth equalities in \eqref{eqn:theorem_dual_15} clearly indicate that in the dual problem \eqref{eqn:dual_operator_5}, one should choose $g = - \Delta e$, and not $g = e$, as we did in \eqref{eqn:theorem_dual_10}, when we proved the $L^2$ error estimate \eqref{eqn:L2Error}.
Using \eqref{eqn:dual_operator_6a} and \eqref{eqn:dual_operator_6c}, the elliptic regularity results of the dual problem \eqref{eqn:dual_operator_5} with $g :=  - \Delta e$, we also get:
\begin{eqnarray}
| \psi^* |_3
\leq C \, | - \Delta e |_{-1}
\leq C \, | e |_1 ,
\label{eqn:theorem_dual_16}
\end{eqnarray}
where in the last inequality we used the fact that $e \in H_0^2(\Omega)$.
Inequality \eqref{eqn:theorem_dual_16} obviously implies
\begin{eqnarray}
| \psi^* |_2
\leq C \, | e |_1 .
\label{eqn:theorem_dual_17}
\end{eqnarray}
All the results in \eqref{eqn:theorem_dual_3}-\eqref{eqn:theorem_dual_7} carry over to our setting.
Thus, we get:
\begin{eqnarray}
|e|_1^2
\leq C \, | e |_2 \, |e^* |_2
+ C \, | e |_2^2 \, | \psi^* |_2 ,
\label{eqn:theorem_dual_18}
\end{eqnarray}
where $C$ is a generic constant that can depend on $Re$, $Ro$, $\Gamma_1$, $\Gamma_2$, $F$, but {\it not} on the meshsize $h$.
By using the approximation result \eqref{eqn:argyris_approximation_2}, we get:
\begin{eqnarray}
|e^* |_2
\leq C \, h \, | \psi^* |_3 .
\label{eqn:theorem_dual_19}
\end{eqnarray}
Inequalities \eqref{eqn:theorem_dual_16}-\eqref{eqn:theorem_dual_19} imply:
\begin{eqnarray}
|e^* |_2
\leq C \, h \, | e |_1 .
\label{eqn:theorem_dual_20}
\end{eqnarray}
Inserting \eqref{eqn:theorem_dual_17} and \eqref{eqn:theorem_dual_20}  in \eqref{eqn:theorem_dual_18}, we get:
\begin{eqnarray}
|e|_1^2
\leq C \, h \, | e |_2 \, | e |_1
+ C \, | e |_2^2 \, | e |_1 .
\label{eqn:theorem_dual_21}
\end{eqnarray}
Using the obvious simplifications and the $H^2$ error estimate \eqref{eqn:H2Error} in \eqref{eqn:theorem_dual_21} yields:
\begin{eqnarray}
|e|_1
\leq C \, h \, | e |_2
+ C \, | e |_2^2
\leq C \, h^5 + C \, h^8
= C_1 \, h^5 ,
\label{eqn:theorem_dual_22}
\end{eqnarray}
which proves the $H^1$ error estimate \eqref{eqn:H1Error}.
%\vspace*{4.0cm}
\hfill
\end{proof}


==> FE.Formulation.tex <==
In this section, we present the functional setting and some auxiliary results for the FEM discretization of the streamfunction formulation of the QGE \eqref{eqn:WeakForm}.
Let $\mathcal{T}^h$ denote a finite element triangulation of $\Omega$ with meshsize (maximum triangle diameter) $h$.
We consider a {\it conforming} FEM discretization of \eqref{eqn:WeakForm}, i.e., $X^h \subset X = H_0^2(\Omega)$.
%A description of the particular finite element we are using (the Argyris triangle) is given at the end of this section (see also Section~\ref{sec:Argyris}).

The FEM discretization of the streamfunction formulation of the QGE \eqref{eqn:WeakForm} reads:
Find $\psi^h \in X^h$ such that 
\begin{eqnarray}
    a_0(\psi^h,\chi^h) + a_1(\psi^h,\psi^h,\chi^h) + a_2(\psi^h,\chi^h) = \ell(\chi^h),\quad \forall \, 
      \chi^h \in X^h.
    \label{eqn:FEForm}
\end{eqnarray}
Using standard arguments \cite{Girault79,Girault86}, one can prove that, if the small data condition used in proving the well-posedness result for the continuous case holds, then \eqref{eqn:FEForm} has a unique solution $\psi^h$ (see Theorem 2.1 in \cite{Cayco86}).
Furthermore, one can prove the following stability result for $\psi^h$ using the same arguments as those used in the proof of Theorem \ref{thm:stability} for the continuous setting.
\begin{theorem} \label{thm:stability_fem}
The solution $\psi^h$ of \eqref{eqn:FEForm} satisfies the following stability estimate:
 \begin{equation}
   |\psi^h|_2 
   \le Re \, Ro^{-1} \, \| F \|_{-2} . 
   \label{eqn:stability_fem_1}
 \end{equation}
\end{theorem}

As noted in Section 6.1 in \cite{Ciarlet} (see also Section 13.2 in \cite{Gunzburger89}, Section 3.1 in \cite{Johnson}, and Theorem 5.2 in \cite{braess2001finite}), in order to develop a conforming FEM for the QGE \eqref{eqn:WeakForm}, we are faced with the problem of constructing subspaces of the space $H^2_0(\Omega)$.
Since the standard, piecewise polynomial FE spaces are locally regular, this construction amounts in practice to finding FE spaces $X^h$ that satisfy the inclusion $X^h \subset C^1({\bar \Omega})$, i.e., finding $C^1$ finite elements.

Several finite elements meet this requirement (see, e.g., Section 6.1 in \cite{Ciarlet}, Section 13.2 in \cite{Gunzburger89}, and Section 5 in \cite{braess2001finite}): the Argyris triangular element, the Bell triangular element, the Hsieh-Clough-Tocher triangular element (a macroelement), and the Bogner-Fox-Schmit rectangular element.
In what follows, we will use the Argyris triangular element, depicted in \autoref{fig:Argyris}.

  \input{Argyris.tex}
  
By using Theorem 6.1.1 and inequality (6.1.5) in \cite{Ciarlet}, we obtain the following two approximation properties for the Argyris FE space $X^h$:
\begin{eqnarray}
\forall \, \chi \in H^6(\Omega) \cap H^2_0(\Omega), \ \exists \, \chi^h \in X^h
\quad \text{such that} \quad
\| \chi - \chi^h \|_2
&\leq& C \, h^4 \, | \chi |_6 ,
\label{eqn:argyris_approximation_0} \\[0.2cm]
\forall \, \chi \in H^4(\Omega) \cap H^2_0(\Omega), \ \exists \, \chi^h \in X^h
\quad \text{such that} \quad
\| \chi - \chi^h \|_2
&\leq& C \, h^2 \, | \chi |_4 ,
\label{eqn:argyris_approximation_1} \\[0.2cm]
\forall \, \chi \in H^3(\Omega) \cap H^2_0(\Omega), \ \exists \, \chi^h \in X^h
\quad \text{such that} \quad
\| \chi - \chi^h \|_2
&\leq& C \, h \, | \chi |_3 ,
\label{eqn:argyris_approximation_2}
\end{eqnarray}
where $C$ is a generic constant that can depend on the data, but not on the meshsize $h$.
Approximation property \eqref{eqn:argyris_approximation_0} follows from inequality (6.1.5) in \cite{Ciarlet} with $q = 2, \, p = 2, \, m = 2$ and $k+1 = 6$.
Approximation property \eqref{eqn:argyris_approximation_1} follows from inequality (6.1.5) in \cite{Ciarlet} with $q = 2, \, p = 2, \, m = 2$ and $k+1 = 4$.
Finally, approximation property \eqref{eqn:argyris_approximation_2} follows from inequality (6.1.5) in \cite{Ciarlet} with $q = 2, \, p = 2, \, m = 2$ and $k+1 = 3$.



==> Future.tex <==
I am writing all the details for now. This is more like a “5-year-plan.” Before
submission, we will of course shorten this significantly. And we will keep our
cards close to the chest, of course. This is for internal use only.

\textbf{Boundary Conditions} I think that we need to be careful when choosing
the BCs. Will the weak formulation change? \textcolor{blue}{Erich: Check this.}
The real issue, however, seems to be the physical relevance of these BCs. In
other words, even though \eqref{eqn:BCs} seems to be popular for error estimates, it
might not be the most physical, say. The paper by Cummins \cite{Cummins} might
be helpful here. Nadiga \emph{et al.}, however, simply uses $\omega = \psi = 0$. We can try to see
whether these BCs give different results from what we get with \eqref{eqn:BCs}.
I think that this could be easily tried in our stationary streamfunction
formulation by using something like $−\Delta \psi = \psi = 0$. Actually, I think
that this is exactly what Dominquez is using in \cite{Dominguez08}.
\textcolor{blue}{Erich: Check this.}

\textbf{Time Discretization} This is very important as a next step. I think this
should be pretty straightforward. Medjo is treating the time-dependent case,
although he does it for the \emph{two-layer} QGE. In \cite{Medjo99}, the
well-posedness of the continuous problem (i.e., no FEM discretization) was
proven. Medjo used a \emph{mixed} variational formulation (that is, he included
the potential vorticity), but he still worked in $H^2$, which makes me wonder
why he did not use the streamfunction formulation. In \cite{Medjo00}, he focused
on the time discretization; he did not talk about the spatial FEM
discretization.

\textbf{Nonconforming FEM}	We should definitely look into applying
nonconforming FEM. Cayco and Nicolaides did just that in \cite{Cayco89} for the
streamfunction formulation of the 2D NSE. I think we could do just the same; the
problem is that it seems that one still has to use some fancy FEM, e.g., Morley
and Fraeijs de Veubeke triangles (see Section 8 in \cite{Cayco89}). \textcolor{blue}{Erich:
Check this.}

\textbf{Conservation Properties} The following paragraph from \cite{Myers} (page
513, top) is illuminating: “Some of the key properties of the FE method applied
to the quasi-geostrophic barotropic vorticity equation were determined by Fix
(1975). He showed that the Galerkin FE method conserved vorticity, energy, and
enstrophy irregardless if any irregularity in the grid and had no hidden
numerical dissipation associated with it. \textcolor{red}{Energy is not
generally conserved in most FD numerical schemes with the exception of the
Arakawa scheme. Even in the Arakawa scheme, enstrophy is only conserved only for
uniform grids and rectangular boundaries.} Fix (1975) also showed that phase
errors are much smaller for the FE method compared to standard FD methods.” 

We should check these conservation properties for the streamfunction formulation
theoretically, just like Fix did for the streamfunction-vorticity formulation.
We should also check them numerically. \textcolor{blue}{Traian, Erich: Can this be
done in the stationary case?}

\textbf{Complex Geometries} Since one of the FEM’s advantages is its ability to
treat complex geometries, it would be really nice to illustrate this
numerically: see, e.g., Figure 1 in \cite{Myers} (showing FDM and FEM domains) and
Figure 8 in \cite{Dijkstra99}. \textcolor{blue}{Traian: Check \cite{Dijkstra05}
for more refs.} It also seems that it would be hard to use the same nice meshes
and geometries as those in [18] without tackling the multiply connected domains
issue (see below).

\textbf{Multiply Connected Domains} Again, the following paragraph from
\cite{Myers} (page 519, subsection d, bottom right) is illuminating:

\textcolor{red}{“Any model that is to be used to study the large-scale ocean
circulation must be capable of dealing with islands.} That is, $\psi$ cannot be
arbitrarily set to zero on island boundaries for this would imply no net
transport between the island and the coast. Instead, a boundary condition of
$\psi = C$ should be used at all boundary points on an island, where $C$ must be
calculated within the model.”

The authors go on to say on page 522, bottom left: “The islands were included in
the domain: Iceland, Ireland, England, ...”

As you can see, these are pretty important islands. Figure 5 on page 523 is
impressive. It would be great if we could do something similar.

Not also that the same holds for NSE. In fact, Max has an entire chapter
(Chapter 12 in \cite{Gunzburger89}) devoted to this issue. Max and Janet also
tackle this issue in \cite{GunzburgerMethods, GunzburgerApprox}.

I think that Tezduyar \emph{et al.} \cite{Tezduyar88, Tezduyar91} also talk about this issue.
\textcolor{blue}{Traian: Check this.}

\textbf{Approximate Deconvolution} Leo should take the lead here. Can any of his
numerical discretizations be used here?

Are the conservation properties valid for the QGE-AD-FEM formulation? (Fix
showed that they are valid in the standard QGE-FEM formulation, without any AD.)

\textbf{F Plane, Two-Layer, and Continuously Stratified QGE} See Majda and Wang
\cite{Majda}. For all these models, we can add AD. Note that Medjo has
\emph{not} used any LES in his two-layer QGE papers. I think that the FEM
analysis is wide open, at least for the F Plane and Continuously Stratified QGE.
\textcolor{blue}{Traian: Check this.} We can also add anisotropic AD, since we
have a vertical component in all these models (note that we don’t have this in
the one-layer QGE, which is 2D).

\textbf{Streamfunction-Vorticity Formulation} This is the other \textbf{major} direction
we should pursue \textbf{in parallel.} Zhu should take the lead here. Leo should get
involved, since this is the formulation he is most comfortable with. It looks
like several authors have used the streamfunction-vorticity ($(\psi, q)$)
formulation. The interesting part is that they all seem to use different
formulations: see \cite{Medjo99, Medjo00} and \cite{Cascon}. I think that the
analysis in \cite{Girault79, Girault86} will be instrumental in deciding what
exactly we need to do. 

Equations (49)-(51) in \cite{Myers} outline the algorithm. \textcolor{blue}{Zhu:
I think this is a good starting point for writing the algorithm and checking the
implementation.}


==> Global.NN.tex <==
\textcolor{red}{Erich: Is this important?  Should we take it out? So what if the matrix is banded?  What advantages does this bring?}
Different node orderings in a mesh correspond to permutations of the stiffness
matrix. 
Since memory use and convergence speed of iterative methods may
depend on the ordering used, it is important to pick a node number that is most
efficient (see, e.g., Fairag \emph{et. al.} \cite{Fairag}). 
The node numbering used in this report is that used in \cite{Fairag}, since it was shown there that it
results in a banded stiffness matrix.

The node ordering consisted of first numbering the vertices of each triangle
with six successive numbers and then numbering the midpoint nodes starting
with the horizontal sides, followed by the vertical and oblique sides. An
illustration of the node numbering can be found in \autoref{fig:MatrixGraph}.
This node numbering results in a banded matrix that can be seen graphically in
\autoref{fig:MatrixGraph}.

\begin{figure}
	\begin{center}
    \begin{tikzpicture}[scale=0.4]
\tikzstyle{every node}=[font=\tiny]
      \draw (0,0) node[below left,fill=none]
      {$\begin{array}{l}1,\\2,3\\4,5,6\end{array}$} 
      -- (3,0) node[below,fill=none] {$25$}
      -- (6,0) node[below right,fill=none]
      {$\begin{array}{l}7,\\8,9\\10,11,12\end{array}$} 
      -- (6,3) node[above right,fill=none] {$29$}
      -- (6,6) node[above right,fill=none] 
      {$\begin{array}{l}19,\\20,21\\22,23,24\end{array}$} 
      -- (3,6) node[above,fill=none] {$26$}
      -- (0,6) node[above left,fill=none]
      {$\begin{array}{l}13,\\14,15\\16,17,18\end{array}$} 
      -- (0,3) node[above left,fill=none] {$27$}
      -- cycle;
      \draw (0,0) -- (3,3) node[above left,fill=none] {$28$} -- (6,6);
    \end{tikzpicture}	
    \hspace*{0.8cm}
    \includegraphics[trim=100 200 100 210, clip, scale=0.35]{Matrix.pdf}
	\end{center}
  \caption{
  Example of element global node numbering (left) and resulting stiffness matrix (right).
  }
	\label{fig:MatrixGraph}
\end{figure}



==> Introduction.tex <==
%\textcolor{blue}{Traian: Finish this}

With the continuous increase in computational power, complex mathematical
models are becoming more and more popular in the numerical simulation of
oceanic and atmospheric flows. For some geophysical flows in which computational
efficiency is of paramount importance, however, simplified mathematical models
are central. 
For example, the \emph{quasi-geostrophic equations (QGE)}, a standard mathematical model for large scale oceanic and atmospheric flows \cite{cushman2011introduction,Majda,Ped92,Vallis06}, are often used in climate modeling \cite{Dijkstra05}.

The QGE are usually discretized in space by using the \emph{finite difference
method} (FDM) \cite{San11}. The \emph{finite element method} (FEM), however, offers several
advantages over the popular FDM, as outlined in \cite{Myers}: (i) an easy treatment of
complex boundaries, such as those of continents for the ocean, or mountains for
the atmosphere; (ii) an easy grid refinement to achieve a high resolution in
regions of interest \cite{Cascon}; (iii) a natural treatment of boundary conditions; and
(iv) a straightforward approach for the treatment of multiply connected domains
\cite{Myers}. Despite these advantages, there are relatively few papers that consider
the FEM applied to the QGE \cite{Cascon,Fix,leprovost1994comparison,Myers,stevens1982finite}.

To our knowledge, {\it all} the {\it finite element (FE)} discretizations of the QGE have been developed for the streamfunction-vorticity formulation, none using the streamfunction formulation.
The reason is simple: The streamfunction-vorticity formulation yields a second order {\it partial differential equation (PDE)}, whereas the streamfunction formulation yields a fourth order PDE.
Thus, although the streamfunction-vorticity formulation has two variables ($q$ and $\psi$) and the streamfunction formulation has just one ($\psi$), the former is the preferred formulation used in practical computations, since its conforming FE discretization requires low-order ($C^0$) elements, whereas the latter requires high-order ($C^1$) elements.

Although the FE discretization of the QGE is relatively scarce, the corresponding error analysis seems to be even more scarce.
To our knowledge, {\it all} the error analysis for the FE discretization of the QGE has been done for the vorticity-streamfunction formulation, and none has been done for the streamfunction formulation.
Furthermore, to the best of our knowledge, all the available error estimates for the FE discretization of the QGE are {\it suboptimal}.
The first error analysis for the FE discretization of the QGE was carried out by Fix \cite{Fix}, in which suboptimal error estimates for the vorticity-streamfunction formulation were proved.
Indeed, relationships (4.7) and (4.8) (and the discussion above these) in \cite{Fix} show that the FE approximations for {\it both} the potential vorticity (denoted by $\zeta$) and streamfunction (denoted by $\psi$) consist of piecewise polynomials of degree $k-1$.
At the top of page 381, the author concludes that the error analysis yields the following estimates:
\begin{eqnarray}
\| \psi - \psi^h \|_1
&=& O(h^{k-1}) ,
\label{eqn:fix_1} \\
\| \zeta - \zeta ^h \|_0
&=& O(h^{k-1}) .
\label{eqn:fix_2}
\end{eqnarray}
Although the streamfunction error estimate \eqref{eqn:fix_1} appears to be optimal, the potential vorticity error estimate \eqref{eqn:fix_2} is clearly suboptimal.
Indeed, using piecewise polynomials of degree $k-1$ for the FEM approximation of the vorticity, one would expect an $O(h^k)$ error estimate in the $L^2$ norm.
Medjo \cite{Medjo99, Medjo00} used a FE discretization of the vorticity-streamfunction formulation and proved error estimates for the time discretization, but no error estimates for the spatial discretization.
Finally, Cascon {\it et al.} \cite{Cascon} proved both {\it a priori} and {\it a posteriori} error estimates for the FE discretization of the {\it linear Stommel-Munk} model (see Section~\ref{sec:Tests} for more details).
This model, while similar to the QGE, has one significant difference: the linear Stommel-Munk model is linear, whereas the QGE is nonlinear.
%Thus, it appears that {\it no optimal} error estimates for the FE discretization of the QGE exist.

We note that the state-of-the-art in the FE error analysis for the QGE seems to reflect that for the {\it two-dimensional Navier-Stokes equations (2D NSE)}, to which the QGE are similar in form. 
Indeed, as carefully discussed in \cite{Gunzburger89} (see also \cite{Fairag98,Fairag03,gunzburger1988finite,gunzburger1988onfinite}), the 2D NSE in streamfunction-vorticity formulation are easy to implement (only $C^0$ elements are needed for a conforming discretization), but the available error estimates are suboptimal (see Section 11.6 in \cite{Gunzburger89}).
Next, we summarize the discussion in \cite{Gunzburger89}, since we believe it sheds light on the QGE setting.
For $C^0$ piecewise polynomial of degree $k$ FE approximation for {\it both} the vorticity (denoted by $\omega$) and streamfunction (denoted by $\psi$), the error estimates given in \cite{Girault86} are (see (11.26) in \cite{Gunzburger89}):
\begin{eqnarray}
| \psi - \psi^h |_1
+ \| \omega - \omega^h \|_0
\leq C \, h^{k - 1/2} \, | \ln h |^{\sigma} ,
\label{eqn:gunzburger_1}
\end{eqnarray}
where $\sigma = 1$ for $k = 1$ and $\sigma = 0$ for $k > 1$.
It is noted in \cite{Gunzburger89} that the error estimate in \eqref{eqn:gunzburger_1} is not optimal: one may loose a half power in $h$ for the derivatives of the streamfunction (i.e., for the velocity), and three-halves power for the vorticity.
It is also noted that there is computational and theoretical evidence that \eqref{eqn:gunzburger_1} is not sharp with respect to the streamfunction error.
Furthermore, in \cite{fix1984mixed} it was shown that, for the {\it linear} Stokes equations, the derivatives of the streamfunction are essentially optimally approximated (see (11.27) in \cite{Gunzburger89}):
\begin{eqnarray}
| \psi - \psi^h |_1
\leq C \, h^{k - \varepsilon} ,
\label{eqn:gunzburger_2}
\end{eqnarray}
where $\varepsilon = 0$ for $k > 1$ and $\varepsilon > 0$ is arbitrary for $k = 1$.
That being said, it is then noted in \cite{Gunzburger89} that  \eqref{eqn:gunzburger_1} seems to be sharp for the vorticity error and thus vorticity approximations are, in general, very poor.

The streamfunction formulation is, from both mathematical and computational points of view, completely different from the vorticity-streamfunction formulation.
Indeed, the FE discretization of the streamfunction formulation generally requires the use of $C^1$ elements (for a conforming discretization), which makes their implementation challenging.
From a mathematical point of view, however, the streamfunction formulation has the following significant advantage over the vorticity-streamfunction formulation: there are optimal error estimates for the FE discretization of the streamfunction formulation (see the error estimate (13.5) and Table 13.1 in \cite{Gunzburger89}), whereas the available error estimates for the vorticity-streamfunction formulation are suboptimal.

The main goal of this paper is twofold. 
First, we use a $C^1$ finite element (the Argyris element) to discretize the streamfunction formulation of the QGE. 
To the best of our knowledge, this is the {\it first} time that a $C^1$ finite element has been used in the numerical discretization of the QGE. 
Second, we derive optimal error estimates for the FE discretization of the QGE and present supporting numerical experiments.
To the best of our knowledge, this is the {\it first} time that optimal error estimates for the QGE have been derived.

The rest of the paper is organized as follows: Section \ref{sec:QGE} presents the QGE, their weak
formulation, and mathematical support for the weak formulation. Section \ref{sec:FEM} outlines the FEM
discretization of the QGE, posing a special emphasis of the Argyris element. Rigorous error
estimates for the FE discretization of the stationary QGE are derived in Section \ref{sec:Errors}.
Several numerical experiments supporting the theoretical results are presented in
Section \ref{sec:NumericalResults}. Finally, conclusions and our future research directions are included in
Section \ref{sec:Conclusions}.


==> Mesh.tex <==
\begin{figure}
	\begin{center}
    \begin{tikzpicture}[scale=0.5]
\tikzstyle{every node}=[font=\tiny]
      \draw (0,0) -- (6,0) -- (6,6) -- (0,6) -- cycle;
      \draw (0,0) -- (6,6);
      \draw (0,3) -- (6,3);
      \draw (3,0) -- (3,6);
      \draw (0,3) -- (3,6);
      \draw (3,0) -- (6,3);
    \end{tikzpicture}
	\end{center}
  \caption{Initial Mesh with $h=0.5$}
	\label{fig:Mesh}
\end{figure}


==> Method.tex <==
The Argyris finite element is implemented for each numerical test (described in
\autoref{sec:Tests}). A discussion of Argyris element was presented in \autoref{sec:FEM}. The
Argyris finite element is implemented on an initial mesh size of $h=\frac{1}{2}$
(\autoref{fig:Mesh}) for each numerical test , and then the mesh is refined by halving the size of
the triangle. The refined results correspond to a mesh size of $h=\frac{1}{4}$.  This process of
mesh refinement is repeated a total of four times resulting in numerical solutions for mesh sizes
corresponding to $h=\left\{\frac{1}{2},\frac{1}{4},\frac{1}{8},\frac{1}{16},\frac{1}{32}\right\}$.
\input{Mesh.tex}

For the numerical tests that are nonlinear, Newton's method is used to solve the resulting
nonlinear system. The stopping criteria for Newton's method is satisfied when the residue and the
two norm of n$^th$ iterate of Newton's method is less than a given tolerance. If we write Newton's
method as 
\begin{equation*}
  \Delta_n \psi^h = -\mathcal{J}(\psi^h_{n-1})^{-1}\, F(\psi^h_{n-1}),
\end{equation*}
where $\Delta_n \psi^h = \psi^h_n - \psi^h_{n-1}$ is the n$^th$ iterate of Newton's method,
$\mathcal{J}(\psi^h_{n-1})$ is the Jacobian matrix evaluated at $\psi^h_{n-1}$, and $F(\psi^h_n-1)$
is the nonlinear problem we are solving evaluated at $\psi^h_{n-1}$ then the residue, $R$ is given by
\begin{equation*}
  R = \left|F(\psi^h_n)\right|
\end{equation*}
where $|\cdot|$ is the one-norm. In addition to the residue and iterate conditions for stopping
criteria Newton's method is required to terminate if a max number of iterations is exceeded. For
each numerical test the max number of iterations for Newton's is set to $100$ and the tolerance is
set to $10^{-8}$.

After the FE code is run for each $h$, the corresponding $\psi^h$ is used to calculate the errors $e_0,\, e_1,\text{
and } e_2$, where $e_0,\, e_1,\text{ and } e_2$ are the $L^2,\, H^1,$ and $H^2$ errors respectively, and are
given by 
%{\small
\begin{align*}
  e_0 &= \left(\int_{\Omega}\!\left( \psi^h - \psi \right)^2 \,d\vec{x}\right)^{\nicefrac{1}{2}}\\
  e_1 &= \left(e_0^2 + \int_{\Omega}\!  \left( \psi^h_x - \psi_x \right)^2 + \left( \psi^h_y - \psi_y \right)^2
    \,d\vec{x}\right)^{\nicefrac{1}{2}}\\
  e_2 &= \left(e_1^2 + \int_{\Omega}\!  \left( \psi^h_{xx} - \psi_{xx} \right)^2 + \left( \psi^h_{xy} - \psi_{xy}
    \right)^2 + \left( \psi^h_{yy} - \psi_{yy} \right)^2 \,d\vec{x}\right)^{\nicefrac{1}{2}}\\
\end{align*}
%}
The order of convergence, $O$, is then determined by calculating 
\begin{equation*}
  O = \dfrac{\log e_{\alpha}^i - \log e_{\alpha}^{i-1}}{\log h_i - \log h_{i-1}},
\end{equation*}
where $e_{\alpha}^i$ is the i$^{th}$ $\alpha$-error corresponding to the i$^{th}$ mesh size, $h_i$. 

Additionally, in each of the convergence data tables we also present the number of degrees of freedom (DoFs) for Argyris
Finite Elements. For the uniform mesh as described above and a rectangular domain of length, $L$, and height, $H$, the
DoFs are given by
\begin{equation*}
  %DoF = 6\cdot\left(\frac{L}{h}+1\right)\cdot\left(\frac{H}{h}+1\right)+\frac{L}{h}\cdot\left(\frac{H}{h}+1\right)+\left(2\frac{L}{h}+1\right)\cdot\frac{H}{h}.
  N = \frac{7h\left(H + L\right) + 9 H L}{h^2} + 6.
\end{equation*}



==> Newton.tex <==
In this section, we briefly outline the implementation details of Newton's method used to solve the nonlinear system of equations resulting from the FE discretization of the streamfunction formulation of the QGE \eqref{eqn:FEForm}.

Newton's method is an iterative process that, at each iteration $n$, with $n=1, 2, \dots$, yields an approximation $\psi^h_n$ to the FEM approximation $\psi^h$.
We start the iterative process by making an initial guess $\psi^h_0$.  
Given $\psi^h_{n-1}$, the Newton iteration at the previous step, Newton's method computes the current step iteration $\psi^h_n$ according to the following formula:
\begin{eqnarray}
  \left(
  \mathcal{J}(\psi^h_{n-1}) \, \Delta_n \psi^h , \chi^h
  \right)
  &=& - 
  \left(
  F(\psi^h_{n-1}) , \chi^h
  \right)
  \qquad
  \forall \, \chi^h \in X^h ,
  \label{eqn:Newton} \\[0.2cm]
  \psi^h_n &=& \Delta_n \psi^h + \psi^h_{n-1},
  \label{eqn:NewPsi}
\end{eqnarray}
where 
\begin{eqnarray*}
  \left(
  F(\psi^h_{n-1}) , \chi^h
  \right)
  &=&  a_0(\psi^h_{n-1},\chi^h) + a_1(\psi^h_{n-1},\psi^h_{n-1},\chi^h) + a_2(\psi^h_{n-1},\chi^h) - \ell(\chi^h), \\[0.2cm]
  \left(
  \mathcal{J}(\psi^h_{n-1}) \, \Delta_n \psi^h , \chi^h
  \right)
  &=& a_0(\Delta_n \psi^h,\chi^h) 
  + a_1(\Delta_n \psi^h,\psi^h_{n-1},\chi^h) 
  \nonumber \\[0.2cm]
  && + a_1(\psi^h_{n-1},\Delta_n \psi^h,\chi^h) 
  + a_2(\Delta_n \psi^h,\chi^h) ,
\end{eqnarray*}
$\mathcal{J}(\psi^h_{n-1})$ is the Jacobian matrix evaluated at $\psi^h_{n-1}$, and
$\Delta_n \psi^h : = \psi^h_n - \psi^h_{n-1}$ is the iteration increment.

In our numerical tests, we use the following stopping criteria for Newton's method:
\begin{eqnarray}
\| R_n \|_{1}
\leq 10^{-8} ,
\label{eqn:newton_stopping_criterion_1} \\
\| \Delta_n \psi^h \|_{2} 
\leq 10^{-8} ,
\label{eqn:newton_stopping_criterion_2} \\
n
\leq 10 ,
\label{eqn:newton_stopping_criterion_3}
\end{eqnarray}
where
\begin{eqnarray}
R_n 
:= \biggl(
F(\psi^h_n) , \varphi^h_i
\biggr)_{i = 1, \ldots, N}
\label{eqn:newton_stopping_criterion_4} 
\end{eqnarray}
is the residual vector at iteration $n$, and $\varphi^h_i, \ i = 1, \ldots, N$, are the FE basis functions.




==> Node.Numbering.tex <==
\begin{figure}
	\begin{center}
    \begin{tikzpicture}[scale=0.4]
\tikzstyle{every node}=[font=\tiny]
      \draw (0,0) node[below left,fill=none]
      {$\begin{array}{l}1,\\2,3\\4,5,6\end{array}$} 
      -- (3,0) node[below,fill=none] {$25$}
      -- (6,0) node[below right,fill=none]
      {$\begin{array}{l}7,\\8,9\\10,11,12\end{array}$} 
      -- (6,3) node[above right,fill=none] {$29$}
      -- (6,6) node[above right,fill=none] 
      {$\begin{array}{l}19,\\20,21\\22,23,24\end{array}$} 
      -- (3,6) node[above,fill=none] {$26$}
      -- (0,6) node[above left,fill=none]
      {$\begin{array}{l}13,\\14,15\\16,17,18\end{array}$} 
      -- (0,3) node[above left,fill=none] {$27$}
      -- cycle;
      \draw (0,0) -- (3,3) node[above left,fill=none] {$28$} -- (6,6);
    \end{tikzpicture}
	\end{center}
  \caption{Global Node Numbering}
	\label{fig:NodeNum}
\end{figure}


==> Normal.Cont.tex <==
\begin{figure}
	\begin{center}
    \begin{tikzpicture}[scale=0.75]
\tikzstyle{every node}=[font=\tiny]
      \draw (0,0) node[below left,fill=none]
      {$\begin{array}{l}1,\\2,3\\4,5,6\end{array}$} 
      -- (3,0) node[below,fill=none] {$37$}
      -- (6,0) node[below right,fill=none]
      {$\begin{array}{l}7,\\8,9\\10,11,12\end{array}$} 
      -- (6,3) node[above right,fill=none] {$42$}
      -- (6,6) node[right,fill=none] 
      {$\begin{array}{l}19,\\20,21\\22,23,24\end{array}$} 
      -- (3,6) node[above left,fill=none] {$38$}
      -- (0,6) node[left,fill=none]
      {$\begin{array}{l}13,\\14,15\\16,17,18\end{array}$} 
      -- (0,3) node[above left,fill=none] {$40$}
      -- cycle;
      \draw (0,0) -- (3,3) node[above left,fill=none] {$41$} -- (6,6);
      \draw (6,6) 
      -- (6,9) node[above right,fill=none] {$45$}
      -- (6,12) node[above right,fill=none] 
      {$\begin{array}{l}31,\\32,33\\34,35,36\end{array}$} 
      -- (3,12) node[above,fill=none] {$39$}
      -- (0,12) node[above left,fill=none]
      {$\begin{array}{l}25,\\26,27\\28,29,30\end{array}$} 
      -- (0,9) node[above left,fill=none] {$43$}
      -- (0,6);
      \draw (0,6) -- (3,9) node[above left,fill=none] {$44$} -- (6,12);
      \draw[<->] (3,7) node[above,fill=none] 
      {$\dfrac{\partial\varphi_{38}}{\partial\vec{n}_{38}}$}
      -- (3,5) node[below,fill=none]
      {$\dfrac{\partial\varphi_{38}}{\partial\vec{n}_{38}}$} ;
    \end{tikzpicture}
	\end{center}
  \caption{Demonstration of Continuity Issue in Normal Derivatives}
	\label{fig:Normals}
\end{figure}


==> Numerical.Test.tex <==
%The main goal of this subsection is twofold. First, we show that the FEM discretization of the
%streamfunction formulation of the QGE \eqref{qge_psi_3} with the Argyris element produces accurate
%numerical approximations. To this end, we benchmark our numerical results against those in the
%published literature \cite{Vallis06, Cascon, Myers}. The second goal is to show that the
%numerical results follow the theoretical error estimates in \autoref{thm:EnergyNorm} and
%\autoref{thm:Errors}, i.e., we compare the observed rates of convergence to the theoretical rates of
%convergence developed in \autoref{sec:Errors}.

\subsection{Mathematical Models}
\label{sec:mathematical_models}

Although the pure streamfunction formulation of the steady QGE \eqref{qge_psi_3} is our main concern,
we also test our Argyris FE discretization on two simplified settings: \begin{inparaenum}[(i)] \item the
\emph{Linear Stommel} model; and \item \emph{Linear Stommel-Munk} model. \end{inparaenum} The reason
for using these two additional numerical tests is that they are standard test problems in the
geophysical fluid dynamics literature (see, e.g., Chapter 13 in Vallis \cite{Vallis06} as well as
the reports of Myers and Weaver \cite{Myers} and Cascon \emph{et al.} \cite{Cascon}). This
allows us to benchmark our numerical results against those in the published literature. Since both
the Linear Stommel and the Linear Stommel-Munk models lack the nonlinearity present in the QGE
\eqref{qge_psi_3}, they represent good stepping stones to verifying our FE discretization.

The \emph{Linear Stommel-Munk} model (see equation (14.42) in \cite{Vallis06} and Problem 2 in \cite{Cascon}) is given by
\begin{equation}
  \epsilon_S \Delta \psi - \epsilon_M \Delta^2 \psi + \frac{\partial \psi}{\partial x} = f,
  \label{eqn:Stommel-Munk}
\end{equation}
where $\epsilon_S \text{ and } \epsilon_M$ are the Stommel number and Munk scale, respectively. The
Stommel number and Munk scale are given by (see, e.g., equation (10) in \cite{Myers} and equations (14.22) and (14.44) in \cite{Vallis06}) 
\begin{eqnarray}
  \epsilon_M = \frac{A}{\beta L^3} \qquad \epsilon_S = \frac{\gamma}{\beta L} 
  \label{eqn:stommel_and_munk_numbers}
\end{eqnarray}
where
$A$ is the eddy viscosity parameterization,
$\beta$ is the coefficient multiplying the $y$ coordinate in the $\beta$-plane approximation \eqref{eqn:beta_plane},
$L$ is the width of the computational domain, and
$\gamma$ is the coefficient of the linear drag (Rayleigh friction) as might be generated by a bottom Ekman layer (see equation (14.5) in \cite{Vallis06}).
The model is
supplemented with appropriate boundary conditions, which will be described for each of the
subsequent numerical tests.

We note that the Linear Stommel-Munk model \eqref{eqn:Stommel-Munk} is similar in form to the QGE
\eqref{qge_psi_3}. Indeed, both models contain the biharmonic operator $\Delta^2 \psi$, the rotation
term $\dfrac{\partial \psi}{\partial x}$, and the forcing term $f$. The two main differences between
the two models are the following: First, the QGE are nonlinear, since they contain the Jacobian term
$J(\psi,q)$, whereas the Stommel-Munk model is linear. The
second difference is that the Linear Stommel-Munk model contains a Laplacian term $\Delta \psi$,
whereas the QGE do not.

We also note that the two models use different parameters: the Reynolds number, $Re$, and the Rossby
number, $Ro$, in \eqref{qge_psi_3} and the Stommel number, $\epsilon_S$, and the Munk scale, $\epsilon_M$,
in the Linear Stommel-Munk model. 
The Munk scale is related to the Rossby and Reynolds numbers by the following relation:
\begin{align}
  \epsilon_M &= Ro\, Re^{-1} . \label{eqn:MunkScale}
\end{align}
There is, however, no explicit relationship between the Stommel number and the Rossby and Reynolds numbers.
The reason is that the QGE \eqref{qge_psi_3} do not contain the Laplacian term that is present in the Stommel-Munk model \eqref{eqn:Stommel-Munk}, which models the bottom Rayleigh friction.
Thus, the coefficient $\gamma$ in \eqref{eqn:stommel_and_munk_numbers} does not have a counterpart in the QGE.
This explains why $\epsilon_S$, which depends on $\gamma$, cannot be directly expressed as a function of $Ro$ and $Re$.

The second simplified model used in our numerical investigation is the \emph{Linear Stommel} model
(equation (14.22) in \cite{Vallis06} and equation (11) in \cite{Myers}):
\begin{equation}
  \epsilon_S \Delta \psi + \frac{\partial \psi}{\partial x} = f.
  \label{eqn:Stommel}
\end{equation}
We note that the Linear Stommel Model \eqref{eqn:Stommel} is just the Linear Stommel-Munk model
\eqref{eqn:Stommel-Munk} in which the biharmonic term is dropped (i.e., $\epsilon_M=0$).




\subsection{Numerical Tests} \label{sec:Tests}

The rest of the subsection is organized as follows: In Section \ref{sss:LSM}, we present results for the
Linear Stommel model \eqref{eqn:Stommel}. In Section \ref{sss:SMM}, we present results for the Linear
Stommel-Munk model \eqref{eqn:Stommel-Munk}. Finally, in Section \ref{sss:SQGE}, we present results for
the (nonlinear) QGE \eqref{qge_psi_3}. 

\subsubsection{Linear Stommel Model} \label{sss:LSM}
This section presents the results for the FEM discretization of the Linear Stommel model
\eqref{eqn:Stommel} by using the Argyris element. The computational domain is $\Omega = [0,1]\times
[0,1]$. For completeness, we present results for two numerical tests. The first test, denoted by
Test 1, corresponds to the exact solution used by Vallis (equation (14.38) in \cite{Vallis06}), while
the second test, denoted by Test 2, corresponds to the exact solution used by Myers \emph{et al.}
(equations (15) and (16) in \cite{Myers}).

\tbf{Test 1a:}
In this test, we choose the same setting as that used by Vallis (equation (14.38) in \cite{Vallis06}).
In particular, the forcing term and the non-homogeneous Dirichlet boundary conditions are chosen to
match those given by the exact solution
\begin{equation}
  \psi(x,y) = (1-x-e^{-\nicefrac{x}{\epsilon_S}}) \sin \pi y
  \label{eqn:MyerExact}
\end{equation}
We choose the same Stommel number as that used by Vallis, i.e., $\epsilon_S=0.04$. The exact solution
\eqref{eqn:MyerExact} considered by Vallis satisfies $\psi \to 0$ as $x \to 0$, but does not vanish
at $x=1$. In our numerical tests, we used a standard lifting procedure to treat these
non-homogeneous boundary conditions.

\autoref{fig:StommelVallis} presents the streamlines of the approximate solution obtained by using
the Argyris Finite Element on a mesh with $h=\frac{1}{32}$ and $9670$ {\it degrees of freedom (DoFs)}. Comparing
\autoref{fig:StommelVallis} with Figure $14.5$ in \cite{Vallis06}, we notice that our approximation
is close to his. Since the exact solution is available, we can compute the errors in various norms.
\autoref{tab:StommelErrorsVallis} presents the errors $e_0,\, e_1, \text{ and } e_2$ (i.e., the
$L^2,\, H^1, \text{ and } H^2$ errors, respectively) for various values of the mesh sizes, $h$ (the
DoFs are also included).

\begin{table}
\begin{center}
{\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $70$ & $0.1148$ & $-$ & $1.81$ & $-$ & $83.67$ & $-$ \\% & $0.00681$ & $-$ \\
  $\nicefrac{1}{4}$ & $206$ & $0.01018$ & $3.495$ & $0.312$ & $2.537$ & $25.48$ & $1.716$ \\% & $0.007801$ & $-0.1961$ \\
  $\nicefrac{1}{8}$ & $694$ & $0.0004461$ & $4.512$ & $0.02585$ & $3.593$ & $3.902$ & $2.707$ \\% & $0.0004681$ & $4.059$ \\
  $\nicefrac{1}{16}$ & $2534$ & $1.09\times 19^{-5}$ & $5.355$ & $0.001215$ & $4.412$ & $0.3494$ & $3.481$ \\% & $1.732\times 19^{-5}$ & $4.756$ \\
  $\nicefrac{1}{32}$ & $9670$ & $1.972\times 19^{-7}$ & $5.788$ & $4.349\times 19^{-5}$ & $4.804$ & $0.02335$ & $3.903$ \\% & $5.396\times 19^{-7}$ & $5.005$ \\
  \hline
\end{tabular}
}
\end{center}
\caption{Linear Stommel Model \eqref{eqn:Stommel}, Test 1 \cite{Vallis06}: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}, especially for the finer meshes.} 
\label{tab:StommelErrorsVallis}
\end{table}

\begin{figure}
  \begin{center}
    \subfigure[Test 1a \cite{Vallis06}] {
      \includegraphics[trim=80 200 70 220, clip=true, scale=0.38]{LinearStommelVallis.pdf}
      \label{fig:StommelVallis}
    }
    \subfigure[Test 1b \cite{Vallis06}: $\epsilon_S=1$.]{
      \includegraphics[trim=80 200 70 220, clip=true, scale=0.38]{StommelVallise1.pdf}
      \label{fig:StommelVallise1}
    }
    \caption{Linear Stommel Model \eqref{eqn:Stommel}: Streamlines of the approximation, $\psi^h$,
    on a mesh size $h = \frac{1}{32}$ and $9670$ DoFs.  Note that our approximation,
    \autoref{fig:StommelVallis}, is close to that of Figure~$14.5$ in
    \cite{Vallis06}.}
    \label{fig:Stommel1}
  \end{center}
\end{figure}
We note that the errors in \autoref{tab:StommelErrorsVallis} follow the theoretical rates of
convergence predicted by the estimates \eqref{eqn:H2Error} - \eqref{eqn:L2Error} in
\autoref{thm:Errors}. The orders of convergence in \autoref{tab:StommelErrorsVallis} are close to
the theoretical ones for the fine meshes, but not as close for the coarse meshes. We think that the
inaccuracies on the coarse meshes are due to their inability to capture the thin boundary layer on
the left-hand side (i.e., at $x=0$). The finer the mesh gets, the better this boundary layer is
captured and the better the numerical accuracy becomes.

\tbf{Test 1b:}
In the Second part of Test 1, we verify the hypothesis above, that is, whether the degrading
accuracy of the approximation is indeed due to the thin (western) boundary layer. To this end, we
change the Stommel number in Test 1a to be $\epsilon_S=1$, which will result in a much thicker western boundary layer. We then run the same numerical test as before, but with the
new Stommel number. As can be seen in \autoref{tab:StommelErrorsVallise1}, the rates of convergence
are the expected theoretical orders of convergence. This shows that the reason for the inaccuracies
in \autoref{tab:StommelErrorsVallis} were indeed due to the thin western boundary layer.

\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $70$ & $1.689\times 10^{-5}$ & $-$ & $0.0003434$ & $-$ & $0.008721$ & $-$ \\%& $4.306\times 10^{-6}$ & $-$ \\
  $\nicefrac{1}{4}$ & $206$ & $3.722\times 10^{-7}$ & $5.504$ & $1.341\times 10^{-5}$ & $4.678$ & $0.0005616$ & $3.957$ \\%& $5.542\times 10^{-7}$ & $2.958$ \\
  $\nicefrac{1}{8}$ & $694$ & $4.891\times 10^{-9}$ & $6.25$ & $3.757\times 10^{-7}$ & $5.158$ & $3.25\times 10^{-5}$ & $4.111$ \\%& $9.043\times 10^{-9}$ & $5.937$ \\
  $\nicefrac{1}{16}$ & $2534$ & $7.079\times 10^{-11}$ & $6.111$ & $1.117\times 10^{-8}$ & $5.071$ & $1.964\times 10^{-6}$ & $4.049$ \\%& $1.355\times 10^{-10}$ & $6.06$ \\
  $\nicefrac{1}{32}$ & $9670$ & $1.08\times 10^{-12}$ & $6.035$ & $3.437\times 10^{-10}$ & $5.023$ & $1.213\times 10^{-7}$ & $4.018$ \\%& $2.169\times 10^{-12}$ & $5.965$ \\
  \hline
\end{tabular}
}
\end{center}
\caption{Linear Stommel Model \eqref{eqn:Stommel}, Test 1b \cite{Vallis06}: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}.} 
\label{tab:StommelErrorsVallise1}
\end{table}
 
\tbf{Test 2:}
For our second test we use the exact solution given by Myers (Equations 15 and 16 in \cite{Myers}), i.e.
{\footnotesize
\begin{equation}
  \psi(x,y) =\frac{\sin(\pi y)}{\pi(1+4\pi^2\epsilon_S^2)}\left\{2\pi\epsilon_S\sin(\pi x)+cos(\pi x)+\frac{1}{e^{R_1}-e^{R_2}}\left[(1+e^{R_2})e^{R_1x}-(1+e^{R_1})e^{R_2x}\right]\right\},
  \label{eqn:MyersExact}
\end{equation}
}
where $R_1\text{ and } R_2$ are the positive and negative roots, respectively, of 
\begin{equation*}
  R = \frac{-1\pm\sqrt{1+4\pi^2 \epsilon_S^2}}{2\epsilon_S}.
\end{equation*}
The forcing term and the homogeneous Dirichlet boundary conditions are chosen to match those given
by the exact solution \eqref{eqn:MyersExact}. We choose the same Stommel number as that used by
Myers, i.e. $\epsilon_S=0.05$.

\autoref{fig:StommelMyers} presents the streamlines of the approximate solution obtained by using the Argyris Finite
Element on a mesh with $h=\frac{1}{32}$ and $9670$ DoFs. Comparing \autoref{fig:StommelMyers} with Figure $2$ in
\cite{Myers}, we notice that our approximation is close to that in \cite{Myers}. Since the exact
solution is available, we can compute the errors in various norms. \autoref{tab:StommelErrorsMyers}
presents the errors $e_0,\, e_1, \text{ and } e_2$ (i.e., the $L^2,\, H^1, \text{ and } H^2$ errors,
respectively) for various values of the mesh sizes, $h$.

\begin{table}
\begin{center}
{\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $70$ & $0.005645$ & $-$ & $0.1451$ & $-$ & $6.602$ & $-$ \\% & $0.0008815$ & $-$ \\
  $\nicefrac{1}{4}$ & $206$ & $0.0004276$ & $3.723$ & $0.02081$ & $2.801$ & $1.632$ & $2.016$ \\% & $0.0003139$ & $1.49$ \\
  $\nicefrac{1}{8}$ & $694$ & $1.46\times 10^{-5}$ & $4.872$ & $0.001408$ & $3.886$ & $0.2066$ & $2.982$ \\% & $2.15\times 10^{-5}$ & $3.868$ \\
  $\nicefrac{1}{16}$ & $2534$ & $2.954\times 10^{-7}$ & $5.627$ & $5.829\times 10^{-5}$ & $4.594$ & $0.0165$ & $3.646$ \\% & $7.097\times 10^{-7}$ & $4.921$ \\
  $\nicefrac{1}{32}$ & $9670$ & $4.968\times 10^{-9}$ & $5.894$ & $1.998\times 10^{-6}$ & $4.867$ & $0.001069$ & $3.948$ \\% & $2.054\times 10^{-8}$ & $5.111$ \\
  \hline
\end{tabular}
}
\end{center}
\caption{Linear Stommel Model \eqref{eqn:Stommel}, Test 2 \cite{Myers}: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}, especially for the finer meshes.} 
\label{tab:StommelErrorsMyers}
\end{table}

\begin{figure}
  \begin{center}
    \includegraphics[trim=80 200 70 220, clip=true, scale=0.38]{LinearStommelMyers.pdf}
    \caption{Linear Stommel Model \eqref{eqn:Stommel}, Test 2 \cite{Myers}: Streamlines of the
    approximation, $\psi^h$, on a mesh size, $h=\frac{1}{32}$, and $9670$ DoFs. Note that our
    approximation is close to that of Figure~$2$ in \cite{Myers}.}
    \label{fig:StommelMyers}
  \end{center}
\end{figure}

We note that the errors in \autoref{tab:StommelErrorsMyers} follow the theoretical rates of convergence predicted by the
estimates \eqref{eqn:H2Error} - \eqref{eqn:L2Error} in \autoref{thm:Errors}. Again, we see that the orders of
convergence in \autoref{tab:StommelErrorsMyers} are close to the theoretical ones for the fine meshes, but not as close
for the coarse meshes. We attribute this to the inaccuracies at the thin (western) boundary layer on the left-hand side (i.e., at
$x=0$). The finer the mesh gets, the better this boundary layer is captured and the better the numerical accuracy becomes.

\subsubsection{Linear Stommel-Munk Model}\label{sss:SMM}
This section presents results for the FEM discretization of the Linear Stommel-Munk model
\eqref{eqn:Stommel-Munk} by using the Argyris element. Our computational setting is the same as that
used by Cascon \emph{et al.} \cite{Cascon}: The computational domain is $\Omega = [0,3]\times[0,1]$,
the Munk scale is $\epsilon_M=6\times 10^{-5}$, the Stommel number is $\epsilon_S=0.05$, and the
boundary conditions are 
\begin{equation} \label{eqn:SMProb}
  \psi = \frac{\partial \psi}{\partial \mathbf{n}}=0 \quad \text{ on } \partial\Omega
\end{equation}
For completeness, we present results for two numerical tests, denoted by Test 3 and Test 4, both
corresponding to Test 1 and Test 2 in \cite{Cascon}, respectively. 

\tbf{Test 3:}
For our third test we use the exact solution given by Test 1 in \cite{Cascon}, i.e.
\begin{equation}
  \psi(x,y) = \sin^2 \frac{\pi x}{3} \sin^2 \pi y.
  \label{eqn:CasconExact1}
\end{equation}
The forcing term is chosen to match that given by the exact solution \eqref{eqn:CasconExact1}.

%For this third test we take $f$ corresponding to applying the linear operator $L$ associated with the \emph{Linear
%Stommel-Munk} model to the exact solution \eqref{eqn:CasconExact1}. 

\autoref{fig:SMsin} presents the streamlines of the approximate solution obtained by using the Argyris Finite
Element on a mesh with $h=\frac{1}{32}$ and $28550$ DoFs. Comparing \autoref{fig:SMsin} with Figure $7$ in
\cite{Myers}, we notice that our approximation is close to that in \cite{Myers}. Since the exact solution is available, we can
compute the errors in various norms. \autoref{tab:SMsinErrors} presents the errors $e_0,\, e_1, \text{ and }
e_2$ (i.e., the $L^2,\, H^1, \text{ and } H^2$ errors, respectively) for various values of the mesh sizes, $h$.

\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $170$ & $0.00299$ & $-$ & $0.04084$ & $-$ & $0.7624$ & $-$ \\%& $0.003423$ & $-$ \\
  $\nicefrac{1}{4}$ & $550$ & $3.217\times 10^{-5}$ & $6.539$ & $0.001031$ & $5.308$ & $0.04078$ & $4.225$ \\%& $1.885\times 10^{-5}$ & $7.505$ \\
  $\nicefrac{1}{8}$ & $1958$ & $3.437\times 10^{-7}$ & $6.548$ & $2.491\times 10^{-5}$ & $5.371$ & $0.002253$ & $4.178$ \\%& $2.371\times 10^{-7}$ & $6.313$ \\
  $\nicefrac{1}{16}$ & $7366$ & $4.571\times 10^{-9}$ & $6.232$ & $7.026\times 10^{-7}$ & $5.148$ & $0.0001344$ & $4.067$ \\%& $4.296\times 10^{-9}$ & $5.786$ \\
  $\nicefrac{1}{32}$ & $28550$ & $6.704\times 10^{-11}$ & $6.091$ & $2.113\times 10^{-8}$ & $5.056$ & $8.26\times 10^{-6}$ & $4.024$ \\%& $6.86\times 10^{-11}$ & $5.969$ \\
 \hline
\end{tabular}
}
\end{center}
\caption{Linear Stommel-Munk Model \eqref{eqn:SMProb}, Test 3 \cite{Cascon}: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}, especially for the finer meshes.} 
\label{tab:SMsinErrors}
\end{table}

\begin{figure}
  \begin{center}
    \subfigure[Test 3 \cite{Cascon}]{
      \includegraphics[trim=80 200 70 220, clip=true, scale=0.38]{StommelMunk1.pdf}
      \label{fig:SMsin}
    }
    \subfigure[Test 4 \cite{Cascon}]{ 
      \includegraphics[trim=80 200 70 220, clip=true, scale=0.38]{StommelMunk2.pdf}
      \label{fig:SMe}
    }
    \caption{Linear Stommel-Munk Model \eqref{eqn:SMProb}: Streamlines of the approximation,
      $\psi^h$, on a mesh size, $h=\frac{1}{32}$, and $28550$ DoFs.  Note that our approximation in
      \autoref{fig:SMsin} and \autoref{fig:SMe} is close to that of Figure $7$ and
      Figure~$10$ in \cite{Cascon}, respectively.}
    \label{fig:StommelMunk}
  \end{center}
\end{figure}

We note that the errors in \autoref{tab:SMsinErrors} follow the theoretical rates of convergence
predicted by the estimates \eqref{eqn:H2Error} - \eqref{eqn:L2Error} in \autoref{thm:Errors}.  This
time, we see that the orders of convergence in \autoref{tab:SMsinErrors} are close to the
theoretical ones for the fine meshes, but are higher than expected for the for the coarse meshes. We
attribute this to the fact that the exact solution \eqref{eqn:CasconExact1} does not display any
boundary layers that could be challenging to capture by the Argyris element on a coarse mesh. 

\tbf{Test 4:}
For our fourth test we use the exact solution given by Test 2 in \cite{Cascon}, i.e.
{\small
\begin{equation}
  \psi(x,y) = \left[\left(1 - \frac{x}{3}\right)\left(1-e^{-20x}\right) \sin \pi y\right]^2.
  \label{eqn:CasconExact2}
\end{equation}
}
Again we take the forcing term $f$ corresponding the exact solution \eqref{eqn:CasconExact2}. 

\autoref{fig:SMe} presents the streamlines of the approximate solution obtained by using the Argyris
Finite Element on a mesh with $h=\frac{1}{32}$ and $28550$ DoFs. Comparing \autoref{fig:SMe} with
Figure $10$ in \cite{Myers}, we notice that our approximation is close to \cite{Myers}. Since the
exact solution is available, we can compute the errors in various norms. \autoref{tab:SMeErrors}
presents the errors $e_0,\, e_1, \text{ and } e_2$ (i.e., the $L^2,\, H^1, \text{ and } H^2$ errors,
respectively) for various values of the mesh sizes, $h$.

\begin{table}
\begin{center}
{\small
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $170$ & $0.06036$ & $-$ & $1.162$ & $-$ & $38.99$ & $-$ \\%& $0.02907$ & $-$ \\
  $\nicefrac{1}{4}$ & $550$ & $0.01132$ & $2.414$ & $0.3995$ & $1.541$ & $21.4$ & $0.8656$ \\%& $0.005678$ & $2.356$ \\
  $\nicefrac{1}{8}$ & $1958$ & $0.0008399$ & $3.753$ & $0.05914$ & $2.756$ & $5.656$ & $1.92$ \\%& $0.0005973$ & $3.249$ \\
  $\nicefrac{1}{16}$ & $7366$ & $2.817\times 10^{-5}$ & $4.898$ & $0.004008$ & $3.883$ & $0.7378$ & $2.939$ \\%& $2.979\times 10^{-5}$ & $4.326$ \\
  $\nicefrac{1}{32}$ & $28550$ & $5.587\times 10^{-7}$ & $5.656$ & $0.0001607$ & $4.641$ & $0.0597$ & $3.627$ \\%& $8.632\times 10^{-7}$ & $5.109$ \\
 \hline
\end{tabular}
}
\end{center}
\caption{Linear Stommel-Munk Model \eqref{eqn:SMProb}, Test 4 \cite{Cascon}: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}, especially for the finer meshes.} 
\label{tab:SMeErrors}
\end{table}

We note that the errors in \autoref{tab:SMeErrors} follow the theoretical rates of convergence
predicted by the estimates \eqref{eqn:H2Error} - \eqref{eqn:L2Error} in \autoref{thm:Errors}. Again,
we see that the orders of convergence in \autoref{tab:SMeErrors} are close to the theoretical ones
for the fine meshes, but not as close for the coarse meshes. As stated previously, we attribute this
to the inaccuracies at the thin (western) boundary layer on the left-hand side (i.e., at $x=0$). The finer the
mesh gets, the better this boundary layer is captured and the better the numerical accuracy becomes.
 
\subsubsection{Quasi-Geostrophic Equations}\label{sss:SQGE}
This section presents results for the FEM discretization of the streamfunction formulation of the
QGE \eqref{qge_psi_3} by using the Argyris element. Our computational domain is
$\Omega=[0,3]\times[0,1]$, the Reynolds number is $Re=1.667$, and the Rossby number is $Ro=10^{-4}$.
For completeness, we present results for two numerical tests, denoted by Test 5 and Test 6, both
corresponding to the exact solutions given in Test 1 and Test 2 of \cite{Cascon}, respectively.

\tbf{Test 5:}
In this test, we take the same exact solution presented in \emph{Test 3}, i.e.
\begin{equation}
  \psi(x,y) = \sin^2 \frac{\pi x}{3} \cdot \sin^2 \pi y.
  \label{eqn:StreamfunctionExact1}
\end{equation}
Again, the forcing term $f$ and homogeneous boundary conditions, $\psi = \frac{\partial
\psi}{\partial \mathbf{n}} = 0$, correspond to the exact solution \eqref{eqn:StreamfunctionExact1}. 

\autoref{fig:SQGEsin} presents the streamlines of the approximate solution obtained by using the
Argyris Finite Element on a mesh with $h=\frac{1}{32}$ and $28550$ DoFs. We note that the
streamlines look as we expect and are similar to those given by Figure $7$ in \cite{Myers}, which
uses the same exact solution.  Since the exact solution is available, we can compute the errors in
various norms. \autoref{tab:SQGEsinErrors} presents the errors $e_0,\, e_1, \text{ and } e_2$ (i.e.,
the $L^2,\, H^1, \text{ and } H^2$ errors, respectively) for various values of the mesh sizes, $h$.

\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $170$ & $0.005709$ & $-$ & $0.06033$ & $-$ & $1.087$ & $-$ \\%& $0.007512$ & $-$ \\
  $\nicefrac{1}{4}$ & $550$ & $3.726\times 10^{-5}$ & $7.259$ & $0.001086$ & $5.796$ & $0.04113$ & $4.724$ \\%& $2.828\times 10^{-5}$ & $8.053$ \\
  $\nicefrac{1}{8}$ & $1958$ & $3.597\times 10^{-7}$ & $6.695$ & $2.534\times 10^{-5}$ & $5.421$ & $0.002252$ & $4.191$ \\%& $3.488\times 10^{-7}$ & $6.341$ \\
  $\nicefrac{1}{16}$ & $7366$ & $4.648\times 10^{-9}$ & $6.274$ & $7.065\times 10^{-7}$ & $5.165$ & $0.0001344$ & $4.067$\\% & $4.696\times 10^{-9}$ & $6.215$ \\
  $\nicefrac{1}{32}$ & $28550$ & $6.737\times 10^{-11}$ & $6.108$ & $2.116\times 10^{-8}$ & $5.061$ & $8.26\times 10^{-6}$ & $4.024$ \\%& $6.965\times 10^{-11}$ & $6.075$ \\
 \hline
\end{tabular}
}
\end{center}
\caption{Full SQGE \eqref{qge_psi_3}, Test 5: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}, especially for the finer meshes.} 
\label{tab:SQGEsinErrors}
\end{table}

\begin{figure}
  \begin{center}
    \subfigure[Test 5 \eqref{eqn:StreamfunctionExact1}]{
      \includegraphics[trim=80 200 70 215, clip=true, scale=0.38]{SQGEsin.pdf}
      \label{fig:SQGEsin}
    }
    \subfigure[Test 6 \eqref{eqn:StreamfunctionExact2}]{
      \includegraphics[trim=80 200 70 215, clip=true, scale=0.38]{SQGEe.pdf}
      \label{fig:SQGEe}
    }
    \caption{Full SQGE \eqref{qge_psi_3}: Streamlines of the approximation, $\psi^h$, on a
    mesh size, $h=\frac{1}{32}$, and $28550$ DoFs.
    }
  \end{center}
\end{figure}

We note that the errors in \autoref{tab:SQGEsinErrors} follow the theoretical rates of convergence
predicted by the estimates \eqref{eqn:H2Error} - \eqref{eqn:L2Error} in \autoref{thm:Errors}. Again,
since the exact solution \eqref{eqn:StreamfunctionExact1} does not display any boundary layers, we
see that the orders of convergence in \autoref{tab:SQGEsinErrors} are close to the theoretical ones for the fine meshes, but are higher
than expected for the for the coarse meshes. 

\tbf{Test 6:}
In this test, we take the same exact solution as used in \emph{Test 4}, i.e.
\begin{equation}
  \psi(x,y) = \left[\left(1 - \frac{x}{3}\right)\left(1-e^{-20x}\right) \sin \pi y\right]^2.
  \label{eqn:StreamfunctionExact2}
\end{equation}
The forcing term $f$ and the homogeneous boundary conditions correspond to the exact solution
\eqref{eqn:StreamfunctionExact2}. 

\autoref{fig:SQGEe} presents the streamlines of the approximate solution obtained by using the
Argyris Finite Element on a mesh with $h=\frac{1}{32}$ and $28550$ DoFs. We note that the
streamlines look as we expect and are similar to those given by Figure $10$ in \cite{Myers}, which
uses the same exact solution. Since the exact solution is available, we can compute the errors in
various norms. \autoref{tab:SQGEeErrors} presents the errors $e_0,\, e_1, \text{ and } e_2$ (i.e.,
the $L^2,\, H^1, \text{ and } H^2$ errors, respectively) for various values of the mesh sizes, $h$.

\begin{table}
\begin{center}
{\small
\begin{tabular}{|c|c|c|c|c|c|c|c|}%c|c|}
  \hline
  $h$ & $DoFs$ & $e_0$ & $L_2$ order & $e_1$ & $H^1$ order & $e_2$ & $H^2$ order \\ % & $e_{\infty}$ & $L_{\infty}$ order \\
  \hline
  $\nicefrac{1}{2}$ & $170$ & $0.3497$ & $-$ & $1.9$ & $-$ & $44.05$ & $-$ \\%& $0.353$ & $-$ \\
  $\nicefrac{1}{4}$ & $550$ & $0.0302$ & $3.533$ & $0.4279$ & $2.15$ & $21.74$ & $1.019$ \\%& $0.03188$ & $3.469$ \\
  $\nicefrac{1}{8}$ & $1958$ & $0.001507$ & $4.324$ & $0.06085$ & $2.814$ & $5.661$ & $1.941$ \\%& $0.002121$ & $3.91$ \\
  $\nicefrac{1}{16}$ & $7366$ & $3.225\times 10^{-5}$ & $5.547$ & $0.004042$ & $3.912$ & $0.7379$ & $2.94$ \\%& $3.832\times 10^{-5}$ & $5.79$ \\
  $\nicefrac{1}{32}$ & $28550$ & $5.672\times 10^{-7}$ & $5.829$ & $0.000161$ & $4.65$ & $0.0597$ & $3.628$ \\%& $8.91\times 10^{-7}$ & $5.426$ \\
 \hline
\end{tabular}
}
\end{center}
\caption{Full SQGE \eqref{qge_psi_3}, Test 6: The errors $e_0,\, e_1,\, e_2$ in the
$L^2,\, H^1,\, H^2$ norms, respectively, for various values of the mesh size, $h$. Note that the orders of convergence
match the theoretical ones in \autoref{thm:Errors}, especially for the finer meshes.} 
\label{tab:SQGEeErrors}
\end{table}

We note that the errors in \autoref{tab:SQGEeErrors} follow the theoretical rates of convergence
predicted by the estimates \eqref{eqn:H2Error} - \eqref{eqn:L2Error} in \autoref{thm:Errors}. Again
for an exact solution which has a western boundary layer, we see that the orders of convergence in \autoref{tab:SQGEeErrors} are close to the theoretical ones for the fine meshes, but
not as close for the coarse meshes. We attribute this to the inaccuracies at the thin boundary layer
on the left-hand side (i.e., at $x=0$). The finer the mesh gets, the better this boundary layer is
captured and the better the numerical accuracy becomes.


==> Numerical.tex <==
In this section we will test the Argyris basis functions and the transformation
that has been developed. This will be done by implementing a finite element
solution to the Biharmonic equation.

Consider the Biharmonic equation in the unit square $\Omega$
\begin{subequations} \label{eqn:problem}
\begin{align}
	\Delta^2 u &= f \text{ on } \Omega \label{eqn:biharmonic}\\
	u= \frac{\partial u}{\partial n} &= 0 \text{ on } \partial \Omega
	\label{eqn:boundary}
\end{align}
\end{subequations}
\subsection{Finite Element Formulation}
Multiplying the left and right of \eqref{eqn:biharmonic} by $v\in
H^{2}_0(\Omega)$ and integrating over $\Omega$ gives
\begin{equation*}
	\int_{\Omega}\! \Delta^2 u v \,dA = \int_{\Omega}\! fv \,dA.
\end{equation*}
Now using the divergence theorem on the left side gives
\eqref{eqn:boundary}
\begin{align*}
	\int_{\Omega}\! \Delta^2 u v \,dA & = \int_{\Omega}\! \nabla \cdot
		\left( \nabla^3 u v \right) - \nabla^3 u \nabla v \,dA \\
  &= \cancelto{0}{\int_{\Delta\Omega}\! \left(\nabla^3 u \cdot \vec{n}\right) v \,dS} -
    \int_{\Omega} \nabla \cdot \left(\Delta u \nabla v\right) - \Delta u \Delta v \,dA \\
  &= \cancelto{0}{\int_{\Delta\Omega}\! \Delta u \frac{dv}{d\vec{n}} \,dS} +
    \int_{\Omega} \Delta u \Delta v \,dA \\
  &= \int_{\Omega} \Delta u \Delta v \,dA.
\end{align*}
Therefore, let 
\begin{align*}
	a(u,v) &= \int_{\Omega}\! \Delta u \Delta v \,dA \\
	\ell(v) &= \int_{\Omega}\! fv \,dA
\end{align*}
and so the problem can be reformulated to 
\begin{equation}
	\begin{split}
	\text{\emph{Find $u \in H^2_0(\Omega)$ such that}}\quad \\ 
	a(u,v) = \ell(v) \quad \forall v \in H^2_0(\Omega).
	\end{split}
\end{equation}
Now let $\mathcal{T}_h$ be the set of non overlapping triangles $K$, and let
$V_h$ be the set of $v_h$ such that $v_h$ is in $\mathbb{P}_5(K)$ and fits the
Argyris criteria in Table ()<++> then $v_h \in H^2(\Omega)$. So,
our problem can be reformulated to
\begin{equation}
	\begin{split}
	\text{\emph{Find $u_h \in H^2_0(\Omega)$ such that}}\quad \\ 
	a(u_h,v_h) = \ell(v_h) \quad \forall v_h \in H^2_0(\Omega).
	\end{split}
\end{equation}

\subsection{Boundary Conditions}
Since the Argyris Element is of type Hermite, we must be careful to satisfy the
boundary conditions. That is, we not only need to force $u=0$ on $\partial
\Omega$, but we me must also force $\nicefrac{\partial u}{\partial
\vec{n}} = 0$ on $\partial \Omega$. 

For the given domain $\Omega=[0,1]\times[0,1]$, we see that along both the lines
$x=0$ and $x=0$ the condition $u=0$ and $\nicefrac{\partial u}{\partial
\vec{n}} = \nicefrac{\partial u}{\partial x}$ implies $\nicefrac{\partial
u}{\partial y} = 0,\; \nicefrac{\partial^2 u}{\partial x \partial y}$ and 
$\nicefrac{\partial^2 u}{\partial y^2}=0$ since $u$ is constant in the $y$
direction on these lines.  Similarly, along the lines $y=0$ and
$y=1$ the conditions $u=0$ and $\nicefrac{\partial u}{\partial \vec{n}} =
\nicefrac{\partial u}{\partial y} = 0$ implies $\nicefrac{\partial
u}{\partial x} = 0,\; \nicefrac{\partial^2 u}{\partial x \partial y}$ and
$\nicefrac{\partial^2 u}{\partial x^2}=0$ since $u$ is constant in the $x$
direction on these lines.

To enforce these boundary conditions the corresponding $u^h_i$ will be set to
zero and only the system containing interior nodes will be considered for the
linear system. For non-rectangular domains things are a bit more complicated,
since linear combinations of $\nicefrac{du}{dx}$ and $\nicefrac{du}{dy}$ will
have to be zero. The linear combination will depend on the direction of the
normal vector $\vec{n}$ corresponding the side of the domain. This more
complicated Neumann boundary condition has not been implemented as of yet, and
so is not considered in the current numerical study.

\subsection{Global Node Numbering}
Different node orderings in a mesh corresponds to permutations of the stiffness
matrix, and since memory use, and convergence speed of iterative methods may
depend on the ordering used it is important to pick a node number that is most
efficient \cite{Fairag}. The node numbering used and that will be
described was taken from Fairag \emph{et. al.}, since they demonstrated that it
resulted in a stiffness matrix that had the desired properties, i.e. a banded
matrix.

The node ordering consisted of first numbering the vertices of each triangle
with six successive numbers and then numbering the midpoint nodes starting,
first, with the horizontal sides, followed by the vertical and oblique sides. An
illustration of the node number can be found in Figure \ref{fig:NodeNum}.

\input{Node.Numbering.tex}

This node numbering resulted in a banded matrix that can be seen graphically in
Figure \ref{fig:MatrixGraph}.

\begin{figure}
	\begin{center}
    \includegraphics[trim=100 235 100 250, clip, scale=0.5]{Matrix.pdf}
	\end{center}
  \caption{Banded Stiffness Matrix as Result of Node Numbering}
	\label{fig:MatrixGraph}
\end{figure}

\subsection{Results}
In our test we take 
\begin{equation}
  u=\left( x\left( x-1 \right)y\left( y-1 \right) \right)^2 
  \label{eqn:u}
\end{equation}
be the exact solution then
\begin{equation}\begin{split}
   f= 8x^2y^2 + 24x^2(x - 1)^2 + 8x^2(y - 1)^2 + 8y^2(x - 1)^2 + 24y^2(y - 1)^2 \\
   + 8(x - 1)^2(y - 1)^2 + 32x(x - 1)*(y - 1)^2 + 32y(y - 1)(x - 1)^2 \\
   + 32xy^2(x - 1) + 32x^2y( y - 1) + 128xy(x - 1)(y - 1)
 \end{split}
   \label{eqn:f}
\end{equation}
To check the code for correctness the rate of convergence in the
$L^2,\,H^1,\text{ and } H^2$ norms were checked. Given the exact solution is $u$
and the approximate solution is $v_{h}$ then the norms are as follows
\begin{align*}
  E_{L^2}(h)=\|u-v_h\|_{L^2} &= \left(\int_{\Omega}\! (u-v_h)^2 \,d\Omega\right)^{\nicefrac{1}{2}}\\
  E_{H^1}(h)=\|u-v_h\|_{H^1} &= \left(\int_{\Omega}\! \sum_{|\alpha|\le 1}
    \left(D^{\alpha}u-D^{\alpha}v_h\right)^2 \,d\Omega\right)^{\nicefrac{1}{2}}\\
  E_{H^2}(h)=\|u-v_h\|_{H^2} &= \left(\int_{\Omega}\! \sum_{|\alpha|\le 2}
    \left(D^{\alpha}u-D^{\alpha}v_h\right)^2 \,d\Omega\right)^{\nicefrac{1}{2}}
\end{align*}
Finally, if $h_i$ is taken to be the mesh size for the current the simulation
then the rate of convergence is taken to be 
\begin{equation*}
  \dfrac{\log(|\nicefrac{E(h_{i-1})}{E(h_i)}|)}{\log(\nicefrac{h_{i-1}}{h_i})} 
\end{equation*}
For our calculations we chose a uniform grid of right isosceles triangles with
leg $h=\{\nicefrac{1}{2},\nicefrac{1}{4},\nicefrac{1}{8},\nicefrac{1}{16}\}$
and the resulting errors and observed rates of convergence can be seen in Table \ref{tab:Errors} 
\begin{table}
  \begin{center}
    \caption{Table of Errors and Observed Rates of Convergence}
{\small
\begin{equation*}
  \begin{array}{|c|c|c|c|c|c|c|}
    \hline
    h & e_2 & L^2\, order & e_{H^1} & H^1\, order &e_{H^2} & H^2\, order \\[0.5em]
    \hline
    0.5 & 6.377\times 10^{-5} & NaN & 5.876\times 10^{-4} & NaN & 9.159\times 10^{-3} & NaN \\[0.5em]
    0.25 & 1.085\times 10^{-6} & 5.878 & 2.607\times 10^{-5} & 4.494 & 7.961\times 10^{-4} & 3.524 \\[0.5em]
    0.125 & 1.24\times 10^{-8} & 6.451 & 6.836\times 10^{-7} & 5.253 & 4.52\times 10^{-5} & 4.139 \\[0.5em]
    0.0625 & 1.434\times 10^{-10} & 6.434 & 1.742\times 10^{-8} & 5.294 & 2.473\times 10^{-6} & 4.192 \\[0.5em]
    \hline
  \end{array}
\end{equation*}}
\end{center}
\label{tab:Errors}
\end{table}
As can be the observed from the table the rate of convergence is seen to be
around $6$ for $L^2$, $5$ for $H^1$, and $4$ for $H^2$ which agree with the
theory.


==> QGE.tex <==
    
The large scale ocean flows, which play a significant role in climate dynamics \cite{Dijkstra05,ghil2008climate}, are driven by two major sources: the wind and the buoyancy (see, e.g., Chapters 14-16 in \cite{Vallis06}).  Winds drive the
subtropical and subpolar gyres, which correspond to the strong, persistent, sub-tropical and
sub-polar western boundary currents in the North Atlantic Ocean (the Gulf Stream and the Labrador
Current) and North Pacific Ocean (the Kuroshio and the Oyashio Currents), as well as their
sub-tropical counterparts in the southern hemisphere \cite{Dijkstra05,Vallis06}.  One of the common
features of these gyres is that they display strong western boundary currents, weak interior
flows, and weak eastern boundary currents.  
%The wind-driven ocean circulation plays a significant
%role in climate dynamics \cite{Dijkstra05,ghil2008climate}.

One of the most popular mathematical models used in the study of large scale wind-driven ocean
circulation is the QGE \cite{cushman2011introduction,Vallis06}.  The QGE represent a simplified model of
the full-fledged equations (e.g., the Boussinesq equations), which allows efficient numerical
simulations while preserving many of the essential features of the underlying large scale ocean
flows.  The assumptions used in the derivation of the QGE include the hydrostatic balance, the
$\beta$-plane approximation, the geostrophic balance, and the eddy viscosity parametrization.
Details of the derivation of the QGE and the approximations used along the way can be found in
standard textbooks on geophysical fluid dynamics, such as
\cite{cushman2011introduction,Maj03,Majda,mcwilliams2006fundamentals,Ped92,Vallis06}. 

In the {\it one-layer QGE}, sometimes called the barotropic vorticity equation, the flow is assumed to be homogenous in the vertical direction. 
Thus, stratification effects are ignored in this model. 
The practical advantages of such a choice are obvious: the computations are two-dimensional, and, thus, the corresponding numerical simulation have a low computational cost.
To include stratification effects, QGE models of increasing complexity have been devised by increasing the number of layers in the model (e.g., the two-layer QGE and the $N$-layer QGE \cite{Vallis06}).
As a first step, in this report we use the one-layer QGE (referred to as ``the QGE" in what follows) to study the wind-driven circulation in an enclosed, midlatitude rectangular basin, which is a standard problem, studied extensively by modelers \cite{cushman2011introduction,Maj03,Majda,mcwilliams2006fundamentals,Ped92,Vallis06}. 

The QGE are usually written as follows (see, e.g., equation (14.57) in \cite{Vallis06}, equation (1.1) in \cite{Majda}, equation (1.1) in \cite{wang1994emergence}, and equation (1) in \cite{greatbatch2000four}): 
\begin{eqnarray}
\frac{\partial q}{\partial t}
+ J(\psi , q)
&=& A \, \Delta q
+ F
\label{qge_q_psi_dim_1} \\
q
&=& \Delta \psi
+ \beta \, y ,
\label{qge_q_psi_dim_2}
\end{eqnarray}
where 
$q$ is the potential vorticity,
$\psi$ is the velocity streamfunction,
$\beta$ is the coefficient multiplying the $y$ coordinate (which is oriented northward) in the $\beta$-plane approximation \eqref{eqn:beta_plane}, 
$F$ is the forcing,
$A$ is the eddy viscosity parametrization, and 
$J(\cdot , \cdot)$ is the Jacobian operator given by
\begin{eqnarray}
J(\psi , q)
:= \frac{\partial \psi}{\partial x} \, \frac{\partial q}{\partial y}
-   \frac{\partial \psi}{\partial y} \, \frac{\partial q}{\partial x} .
\label{eqn:jacobian}
\end{eqnarray}
The $\beta$-plane approximation reads
\begin{eqnarray}
f
= f_0
+ \beta \, y ,
\label{eqn:beta_plane}
\end{eqnarray}
where 
$f$ is the Coriolis parameter and 
$f_0$ is the reference Coriolis parameter 
(see, e.g., \cite{cushman2011introduction} or Section 2.3.2 in \cite{Vallis06}).

As noted in Section 10.7.2 in \cite{Vallis06} (see also \cite{san2012approximate}), the eddy viscosity parameter $A$ in \eqref{qge_q_psi_dim_1} is usually significantly higher than the molecular viscosity.
This choice allows the use of a coarse mesh in numerical simulations. 
The horizontal velocity ${\bf u}$ can be recovered from $\psi$ and $q$ by using the following formula:
\begin{eqnarray}
{\bf u}
:= \nabla^{\perp} \psi
= \left(
\begin{array}{c}
- \frac{\partial \psi}{\partial y} \\[0.2cm]
\ \ \frac{\partial \psi}{\partial x}
\end{array}
\right) .
\label{eqn:u_psi}
\end{eqnarray}

The computational domain is standard \cite{greatbatch2000four}, a rectangular, closed basin on a $\beta$-plane with the $y$ coordinate increasing northward and the $x$ coordinate eastward.
The center of the basin is at $y=0$, the northern and southern boundaries are at $y = \pm \, L$, respectively, and the western and eastern boundaries are at $x = 0$ and $x = L$ (see Figure 1 in \cite{greatbatch2000four}).

We are now ready to nondimensionalize the QGE \eqref{qge_q_psi_dim_1}-\eqref{qge_q_psi_dim_2}.
There are several ways of nondimensionalizing the QGE, based on different scalings and involving different parameters (see standard textbooks, such as \cite{cushman2011introduction,Majda,Ped92,Vallis06}).
Since the FEM error analysis in this report is based on a precise relationship among the nondimensional parameters of the QGE (see, e.g., \eqref{eqn:small_data_condition}), we present below a careful nondimensionalization of the QGE.

We first need to choose a length scale and a velocity scale.
The length scale we choose is $L$, the width of the computational domain.
The velocity scale is the Sverdrup velocity
\begin{eqnarray}
U
:= \frac{\pi \, \tau_0}{\rho \, H \, \beta \, L} ,
\label{eqn:velocity_scale}
\end{eqnarray}
where 
$\tau_0$ is the amplitude of the wind stress,
$\rho$ is the density of the fluid, and
$H$ is the height of the fluid.
The Sverdrup balance, which was used in the derivation of \eqref{eqn:velocity_scale}, expresses the balance between the two dominant effects in the system: the $\beta$-effect and the curl of the divergence of the wind stress (see, e.g., Section 14.1.3 in \cite{Vallis06}).
Once the length and velocity scales are chosen, the variables in the QGE \eqref{qge_q_psi_dim_1}-\eqref{qge_q_psi_dim_2} can be nondimensionalized as follows:
\begin{eqnarray}
x^*
= \frac{x}{L}, 
\quad
y^*
= \frac{y}{L}, 
\quad
t^*
= \frac{t}{L / U},
\quad
q^*
= \frac{q}{\beta \, L},
\quad
\psi^*
= \frac{\psi}{U \, L} ,
\label{eqn:nondimensional_variables}
\end{eqnarray}
where a $^*$ superscript denotes the nondimensional variable.
We first nondimensionalize \eqref{qge_q_psi_dim_2}.
Using \eqref{eqn:nondimensional_variables}, \eqref{qge_q_psi_dim_2} becomes
\begin{eqnarray}
\beta \, L \, q^*
= \frac{1}{L^2} \, \Delta^* (U \, L \, \psi^*)
+ \beta \, (L \, y^*) .
\label{qge_q_psi_nondim_1}
\end{eqnarray}
Dividing \eqref{qge_q_psi_nondim_1} by $\beta \, L$, we get:
\begin{eqnarray}
q^*
= \left( \frac{U}{\beta \, L^2} \right) \, \Delta^* \psi^*
+ y^* .
\label{qge_q_psi_nondim_2}
\end{eqnarray}
Defining the {\it Rossby number, $Ro$,} as follows
\begin{eqnarray}
Ro
:= \frac{U}{\beta \, L^2} ,
\label{eqn:rossby_number}
\end{eqnarray}
equation \eqref{qge_q_psi_nondim_2} becomes
\begin{eqnarray}
q^*
= Ro \, \Delta^* \psi^*
+ y^* .
\label{qge_q_psi_nondim_3}
\end{eqnarray}

We note that all the nondimensionalizations in \eqref{eqn:nondimensional_variables} are naturally based on the velocity scale, $U$, and the length scale, $L$, except $q^*$. 
Indeed, a nondimensionalization of the form
\begin{eqnarray}
{\tilde q}
= \frac{U}{L},
\label{eqn:qge_q_psi_nondim_4}
\end{eqnarray}
would probably be more natural.
Note that the alternative nondimensionalization in \eqref{eqn:qge_q_psi_nondim_4} is indeed correct, i.e., the variable ${\tilde q}$ is nondimensional.
The main reason for which the nondimensionalization in \eqref{eqn:nondimensional_variables} is used instead the one in \eqref{eqn:qge_q_psi_nondim_4} is that the former yields just one constant (the Rossby number $Ro$) in \eqref{qge_q_psi_nondim_3}, whereas the latter would yield two constants.

Next, we nondimensionalize \eqref{qge_q_psi_dim_1}.
We start with the left-hand side:
\begin{eqnarray}
\frac{\partial q}{\partial t}
&=& ( \beta \, U) \, \frac{\partial q^*}{\partial t^*} ,
\label{eqn:qge_q_psi_nondim_5} \\[0.2cm]
J(\psi,q)
&=&  \frac{\partial \psi}{\partial x} \, \frac{\partial q}{\partial y}
  -     \frac{\partial \psi}{\partial y} \, \frac{\partial q}{\partial x}
=     U \, \frac{\partial \psi^*}{\partial x^*} \, \beta \, \frac{\partial q^*}{\partial y^*}
  -    U \, \frac{\partial \psi^*}{\partial y^*} \,  \beta \, \frac{\partial q^*}{\partial x^*}
\nonumber \\[0.2cm]
&=& (  \beta \, U ) \, J^*(\psi^*,q^*) .
\label{eqn:qge_q_psi_nondim_6}
\end{eqnarray}

Next, we nondimensionalize the right-hand side of \eqref{qge_q_psi_dim_1}.
The first term can be nondimensionalized as follows:
\begin{eqnarray}
A \, \Delta q
&=& A \, \left( \frac{\partial^2 q}{\partial x^2} 
+ \frac{\partial^2 q}{\partial y^2} \right)
%\nonumber \\[0.2cm]
%&=& 
= A \,  \left( 
    \frac{1}{L^2} \, \frac{\partial^2}{\partial {x^*}^2} \, (\beta \, L \, q^*)
+  \frac{1}{L^2} \, \frac{\partial^2}{\partial {y^*}^2} \, (\beta \, L \, q^*)
\right)
\nonumber \\[0.2cm]
&=& A \, \frac{\beta}{L} \, \Delta^* q^* .
\label{eqn:qge_q_psi_nondim_7}
\end{eqnarray}
Thus, inserting \eqref{eqn:qge_q_psi_nondim_5}-\eqref{eqn:qge_q_psi_nondim_7} in \eqref{qge_q_psi_dim_1}, we get:
\begin{eqnarray}
 ( \beta \, U) \, \frac{\partial q^*}{\partial t^*}
+ (  \beta \, U ) \, J^*(\psi^*,q^*)
&=& A \, \frac{\beta}{L} \, \Delta^* q^*
+ F .
\label{eqn:qge_q_psi_nondim_8}
\end{eqnarray}
Dividing by $\beta \, U$, we get:
\begin{eqnarray}
\frac{\partial q^*}{\partial t^*}
+ J^*(\psi^*,q^*)
&=& \left( \frac{A}{U \, L} \right) \, \Delta^* q^*
+ \frac{F}{\beta \, U} .
\label{eqn:qge_q_psi_nondim_9}
\end{eqnarray}
Defining the {\it Reynolds number, $Re$,} as follows
\begin{eqnarray}
Re
:= \frac{U \, L}{A} ,
\label{eqn:reynolds_number}
\end{eqnarray}
equation \eqref{eqn:qge_q_psi_nondim_9} becomes
\begin{eqnarray}
\frac{\partial q^*}{\partial t^*}
+ J^*(\psi^*,q^*)
&=& Re^{-1} \, \Delta^* q^*
+ \frac{F}{\beta \, U} .
\label{eqn:qge_q_psi_nondim_10}
\end{eqnarray}
As noted above, the Sverdrup balance expresses the balance between the two dominant effects in the system: the $\beta$-effect and the curl of the divergence of the wind stress (see, e.g., Section 14.1.3 in \cite{Vallis06}).
The velocity scale, $U$, in \eqref{eqn:velocity_scale} was chosen according to the Sverdrup balance.
Thus, the last term on the right-hand side of \eqref{eqn:qge_q_psi_nondim_10} has the following units:
\begin{eqnarray}
\left[ \frac{F}{\beta \, U} \right]
\sim \left[ \frac{\frac{\nabla \times (\nabla \cdot \tau_0)}{\rho}}{\beta \, U}  \right]
\stackrel{\eqref{eqn:velocity_scale}}{\sim} 
\left[ \frac{\frac{\nabla \times (\nabla \cdot \tau_0)}{\rho}}{\frac{\pi \, \tau_0}{\rho \, H \, L}}  \right] ,
\label{eqn:qge_q_psi_nondim_11}
\end{eqnarray}
which, after the obvious simplification, is clearly nondimensional.
Thus, \eqref{eqn:qge_q_psi_nondim_11} clearly shows that the last term on the right-hand side of \eqref{eqn:qge_q_psi_nondim_10} is nondimensional, so \eqref{eqn:qge_q_psi_nondim_10} becomes:
\begin{eqnarray}
\frac{\partial q^*}{\partial t^*}
+ J^*(\psi^*,q^*)
&=& Re^{-1} \, \Delta^* q^*
+ F^* ,
\label{eqn:qge_q_psi_nondim_12}
\end{eqnarray}
where
\begin{eqnarray}
F^* 
:= \frac{F}{\beta \, U} .
\label{eqn:qge_q_psi_nondim_12b}
\end{eqnarray}




==> Streamfunction.tex <==
Dropping the $^*$ superscript in \eqref{qge_q_psi_nondim_3} and \eqref{eqn:qge_q_psi_nondim_12}, we obtain the nondimensional {\it vorticity-streamfunction formulation} of the {\it one-layer quasi-geostrophic equations}
\begin{eqnarray}
\frac{\partial q}{\partial t}
+ J(\psi , q)
&=& Re^{-1} \, \Delta q
+ F
\label{qge_q_psi_1} \\
q
&=& Ro \, \Delta \psi
+ y ,
\label{qge_q_psi_2}
\end{eqnarray}
where $Re$ and $Ro$ are the Reynolds and Rossby numbers defined in \eqref{eqn:reynolds_number} and \eqref{eqn:rossby_number}, respectively.
%\textcolor{blue}{Traian: Make sure you define $Re$ and $Ro$.}
The stationary QGE are obtained by setting $\displaystyle \frac{\partial q}{\partial t}$ to $0$ in \eqref{qge_q_psi_1}.
\begin{eqnarray}
J(\psi , q)
&=& Re^{-1} \, \Delta q
+ F
\label{qge_q_psi_3} \\
q
&=& Ro \, \Delta \psi
+ y .
\label{qge_q_psi_4}
\end{eqnarray}
Substituting \eqref{qge_q_psi_4} in \eqref{qge_q_psi_3} and dividing by $Ro$, we get the {\it streamfunction formulation} of the {\it one-layer quasi-geostrophic equations}
\begin{eqnarray}
- Re^{-1} \, \Delta^2 \psi 
+ J(\psi , \Delta \psi)
+ Ro^{-1} \, \frac{\partial \psi}{\partial x}
= Ro^{-1} \, F .
\label{qge_psi_1}
\end{eqnarray}

Equations \eqref{qge_q_psi_3}-\eqref{qge_q_psi_4} and \eqref{qge_psi_1} are the usual formulations of the steady, one-layer QGE in streamfunction-vorticity and streamfunction formulations, respectively.
We note that the streamfunction-vorticity formulation has two unknowns ($q$ and $\psi$), whereas the streamfunction formulation has only one unknown ($\psi$).
%The streamfunction-vorticity formulation, however, is more popular than the streamfunction formulation, since the former is a second-order PDE, whereas the latter is a fourth-order PDE.
Because the streamfunction-vorticity formulation  is a second-order PDE, whereas the streamfunction formulation is a fourth-order PDE, the former is more popular in practical computations.

We also note that \eqref{qge_q_psi_3}-\eqref{qge_q_psi_4} and \eqref{qge_psi_1} are similar in form to the 2D NSE written in the streamfunction-vorticity and streamfunction formulations, respectively.
Indeed, \eqref{qge_q_psi_3}-\eqref{qge_q_psi_4} and \eqref{qge_psi_1} are almost the same as (11.3)-(11.4) and (13.1) in \cite{Gunzburger89}, which are obtained by first writing 
\begin{eqnarray}
{\bf u}
= \left(
\begin{array}{c}
\ \ \frac{\partial \psi}{\partial y} \\[0.2cm]
- \frac{\partial \psi}{\partial x}
\end{array}
\right)
\label{qge_psi_2}
\end{eqnarray}
and then taking the curl of the 2D NSE.
There are, however, several significant differences between the QGE and the 2D NSE.
First, we note that the term $y$ in \eqref{qge_q_psi_4} and the corresponding term $\displaystyle \frac{\partial \psi}{\partial x}$ in \eqref{qge_psi_1}, which model the {\it rotation effects} in the QGE, do not have counterparts in the 2D NSE.
Furthermore, the Rossby number, $Ro$, in the QGE, which is a measure of the rotation effects, does not appear in the 2D NSE.
Apart from these two significant differences, however, the streamfunction-vorticity and streamfunction formulations of the QGE and the 2D NSE are quite similar.
Thus, for notation consistency (i.e., to ensure that the velocity and the streamfunction are related by \eqref{qge_psi_2}, which is just \eqref{eqn:u_psi} with a changed sign), we will consider the QGE \eqref{qge_psi_1} with $\psi$ replaced by $- \psi$:
\begin{eqnarray}
Re^{-1} \, \Delta^2 \psi 
+ J(\psi , \Delta \psi)
- Ro^{-1} \, \frac{\partial \psi}{\partial x}
= Ro^{-1} \, F .
\label{qge_psi_3}
\end{eqnarray}

At this point, let us comment on the significance of the two parameters in \eqref{qge_psi_3}, the Reynolds number, $Re,$ and the Rossby number, $Ro$.
As in the 2D NSE case, $Re$ is the coefficient of the diffusion term $- \Delta q = \Delta^2 \psi$.
The higher $Re$, the smaller the magnitude of the diffusion term as compared with the nonlinear convective term $- J(\psi, \Delta \psi) = ( \nabla \psi^{\perp} \cdot \nabla ) q = ({\bf u} \cdot \nabla ) q$.
Since the parameter $Ro$, quantifying the rotation effects in the QGE, does not appear in the 2D NSE, its significance deserves a special attention.
We first note that, for small $Ro$, which corresponds to large rotation effects, the forcing term, $Ro^{-1} \, F$, becomes large compared with the other terms.
But probably the most interesting term in \eqref{qge_psi_3} is $\displaystyle Ro^{-1} \, \frac{\partial \psi}{\partial x}$, which could be interpreted as a convection type term with respect to $\psi$, not to $q = -\Delta \psi$.
When $Ro$ is small, $\displaystyle Ro^{-1} \, \frac{\partial \psi}{\partial x}$ becomes large. 
In conclusion, the physically relevant cases for large scale oceanic flows, in which $Re$ is large and $Ro$ is small (i.e., small diffusion and high rotation, respectively) translate mathematically into a {\it convection-dominated} PDE with {\it large forcing}.
Thus, from a mathematical point of view, we expect the restrictive conditions used to prove the well-posedness of the 2D NSE \cite{Girault79,Girault86,Gunzburger89} to be even more restrictive in the QGE setting, due to the rotation effects.
We will later see that this is indeed the case.

To completely specify the equations in \eqref{qge_psi_3}, we need to impose boundary conditions. 
The question of appropriate boundary conditions for the QGE is a thorny one, especially for the vorticity-streamfunction formulation (see \cite{Vallis06,Cummins} for a careful discussion of this issue).
In this report, we consider 
\begin{eqnarray}
\psi 
= \frac{\partial \psi}{\partial {\bf n}}
= 0
\qquad
\text{on } \partial \Omega,
\label{qge_psi_4}
\end{eqnarray}
which are also the boundary conditions used in \cite{Gunzburger89} for the streamfunction formulation of the 2D NSE.



==> Weak.Formulation.tex <==
We are now ready to derive the weak formulation of the QGE in streamfunction formulation \eqref{qge_psi_3}.
To this end, we first introduce the appropriate functional setting.
Let
\begin{equation*}
  X 
  := H^2_0(\Omega) 
  = \left\{ \psi\in H^2(\Omega):
    \psi=\frac{\partial\psi}{\partial {\bf n}}=0 \text{ on } \partial\Omega \right\} .
\end{equation*}
Multiplying \eqref{qge_psi_3} by a test function $\chi \in X$ and using the divergence theorem, we get, in a standard way (see \cite{Gunzburger89}), the {\it weak formulation} of the QGE in streamfunction formulation:
\begin{eqnarray}
&& Re^{-1} \, \int_{\Omega} \, \Delta \psi \, \Delta \chi \, d{\bf x}
+ \int_{\Omega} \, \Delta \psi \, \left( \psi_y \, \chi_x - \psi_x \, \chi_y \right) \, d{\bf x}
- Ro^{-1} \, \int_{\Omega} \, \psi_x \, \chi \, d{\bf x} 
\nonumber \\
&& \hspace*{3.0cm} = Ro^{-1} \, \int_{\Omega} \, F \, \chi \, d{\bf x} 
\qquad \forall \, \chi \in X .
\label{eqn:qge_psi_weak}
\end{eqnarray}
Therefore, letting
\begin{align}
  a_0(\psi,\chi) &= Re^{-1} \, \int_{\Omega} \, \Delta \psi \, \Delta \chi \, d{\bf x} , \label{eqn:a0} \\
  a_1(\zeta,\psi,\chi) &= \int_{\Omega} \, \Delta \zeta \, \left( \psi_y \, \chi_x - \psi_x \, \chi_y \right) \, d{\bf x} , \label{eqn:a1} \\
  a_2(\psi,\chi) &= - Ro^{-1} \, \int_{\Omega} \, \psi_x \, \chi \, d{\bf x} , \label{eqn:a2} \\
  \ell(\chi) &= Ro^{-1} \, \int_{\Omega} \, F \, \chi \, d{\bf x} , \label{eqn:l}
\end{align}
gives the following weak formulation of the QGE in streamfunction formulation: Find $\psi \in X$ such that
\begin{equation}
    a_0(\psi,\chi) + a_1(\psi,\psi,\chi) + a_2(\psi,\chi) = \ell(\chi),\quad \forall
      \chi \in X.
    \label{eqn:WeakForm}
\end{equation}
The linear form $\ell$, the bilinear forms $a_0$ and $a_2$, and the trilinear
form $a_1$ are continuous: There exist $\Gamma_1 > 0$ and $\Gamma_2 > 0$ such that 
\begin{align}
  | a_0(\psi,\chi) | &\le Re^{-1} \,  |\psi|_2 \, |\chi|_2 \quad \forall \, \psi,\chi\in X , \label{eqn:a0Cont} \\
  | a_1(\zeta,\psi,\chi) | &\le \Gamma_1 \, |\zeta|_2 \, |\psi|_2 \, |\chi|_2 \quad \forall \, \zeta,\psi,\chi\in X , \label{eqn:a1cont} \\
  | a_2(\psi,\chi) | &\le Ro^{-1} \, \Gamma_2 \, |\psi|_2 \, |\chi|_2 \quad \forall \, \psi, \, \chi \in X , \label{eqn:a2Cont} \\
  | \ell(\chi) | &\le Ro^{-1} \,\|F\|_{-2} \, |\chi|_2 \quad \forall \, \chi \in X . \label{eqn:lCont}
\end{align}
Inequalities \eqref{eqn:a0Cont}, \eqref{eqn:a1cont}, and \eqref{eqn:lCont} are stated in \cite{Cayco86} (see inequalities (2.2) and (2.3) in  \cite{Cayco86}).
Inequality \eqref{eqn:a2Cont} can be proved as follows.
Proposition 2.1(iii) in \cite{Medjo99} implies that 
\begin{eqnarray}
| a_2(\psi,\chi) | 
\le Ro^{-1} \,C \, \|\psi\|_2 \, \|\chi\|_2 ,
\label{eqn:medjo}
\end{eqnarray}
where $C$ is a generic constant.
Theorem 1.1 in \cite{Girault86} implies that $| \cdot |_2$, the $H^2$-seminorm, and $\| \cdot \|_2$, the $H^2$-norm are equivalent on $X = H_0^2$.
Thus, \eqref{eqn:medjo} yields inequality \eqref{eqn:a2Cont}.


==> WellPosed.tex <==

For small enough data, one can use the same type of arguments as in \cite{Girault79,Girault86} to prove that the QGE in streamfunction formulation \eqref{eqn:WeakForm} are well-posed \cite{barcilon1988existence,wolansky1988existence}.
In what follows, we will always assume that the small data condition involving $Re$, $Ro$ and $F$, is satisfied and, thus, that there exists a unique solution $\psi$ to \eqref{eqn:WeakForm}.

Using a standard argument (see Theorem 2.1 in \cite{Cayco86}), one can also prove the following stability estimate:
\begin{theorem} \label{thm:stability}
The solution $\psi$ of \eqref{eqn:WeakForm} satisfies the following stability estimate:
 \begin{equation}
   |\psi|_2 
   \le Re \, Ro^{-1} \, \| F \|_{-2} . 
   \label{eqn:stability_1}
 \end{equation}
\end{theorem}
\begin{proof}
Setting $\chi = \psi$ in \eqref{eqn:WeakForm}, we get:
\begin{eqnarray}
a_0(\psi, \psi) 
+ a_1(\psi,\psi, \psi) 
+ a_2(\psi, \psi) 
= \ell(\psi) .
\label{eqn:stability_2}
\end{eqnarray}
Since the trilinear form $a_1$ is skew-symmetric in the last two arguments \cite{Girault79,Girault86,Gunzburger89}, we have
\begin{eqnarray}
a_1(\psi,\psi, \psi) 
= 0 .
\label{eqn:stability_3}
\end{eqnarray}
We also note that, applying Green's theorem, we have
\begin{eqnarray}
a_2(\psi,\psi) 
&=& - Ro^{-1} \, \iint_{\Omega} \frac{\partial \psi}{\partial x} \, \psi \, dx \, dy 
%\nonumber \\
%&=& 
\, = \, - \frac{Ro^{-1}}{2} \, \iint_{\Omega} \frac{\partial}{\partial x} (\psi^2) \, dx \, dy \nonumber \\
&=& - \frac{Ro^{-1}}{2} \, \iint_{\Omega} \left( \frac{\partial}{\partial x} (\psi^2) 
- \frac{\partial}{\partial y} (0) \right) \, dx \, dy 
%\nonumber \\
%&=& 
\, = \, - \frac{Ro^{-1}}{2} \, \int_{\partial \Omega} 0 \, dx + \psi^2 \, dy \nonumber \\
&=& 0 ,
\label{eqn:stability_4}
\end{eqnarray}
where in the last equality in \eqref{eqn:stability_4} we used that $\psi = 0$ on $\partial \Omega$ (since $\psi \in H_0^2(\Omega)$).
Substituting \eqref{eqn:stability_4} and \eqref{eqn:stability_3} in \eqref{eqn:stability_2} and using the Cauchy-Schwarz inequality, we get:
\begin{eqnarray}
| \psi |_{2}^2
= \int_{\Omega} \Delta \psi \, \Delta \psi \, d{\bf x}
= Re \, Ro^{-1} \, \int_{\Omega} F \, \psi \, d{\bf x}
\leq Re \, Ro^{-1} \, \| F \|_{-2} \, | \psi |_{2} ,
\label{eqn:stability_5}
\end{eqnarray}
which proves \eqref{eqn:stability_2}.
\hfill
\end{proof}


==> conclusions.tex <==
This paper introduced a conforming finite element discretization of the streamfunction formulation of the stationary one-layer quasi-geostrophic equations based on the Argyris element. 
For this finite element discretization, we proved optimal error estimates in the $H^2$, $H^1$ and $L^2$ norms.
A careful numerical investigation of the finite element discretization was also performed.
To this end, the quasi-geostrophic equations as well as the linear Stommel and Stommel-Munk models (two standard simplified settings used in the geophysical fluid dynamics literature \cite{Vallis06,Myers,Cascon}) were used in the numerical tests.
Based on the numerical results from the six tests considered, we drew the following two conclusions: (i) our numerical results are close to those used in the published literature \cite{Vallis06,Myers,Cascon}; and (ii) the convergence rates of the numerical approximations do indeed follow the theoretical error estimates in Theorems \ref{thm:EnergyNorm} and \ref{thm:Errors}.
The convergence rates followed exactly the theoretical ones in the test problems where the exact solution did not display a thin boundary layer, but where somewhat lower than expected in those tests that displayed a thin western boundary layer, as expected.

We plan to extend this study in several directions, including the time-dependent quasi-geostrophic equations and the two-layer quasi-geostrophic equations.



==> numerical_results.tex <==
The main goal of this section is twofold. First, we show that the FE discretization of the
streamfunction formulation of the QGE \eqref{eqn:FEForm} with the Argyris element produces accurate
numerical approximations. To this end, we benchmark our numerical results against those in the
published literature \cite{Cascon,Myers,Vallis06}. The second goal of this section is to show that
the numerical results follow the theoretical error estimates in \autoref{thm:EnergyNorm} and
\autoref{thm:Errors}.

The rest of the section is organized as follows.
In Section \ref{sec:Newton}, we briefly describe the implementation details of the Newton method used to solve the nonlinear system of equations resulting from the FEM discretization of the streamfunction formulation of the QGE \eqref{eqn:FEForm}.
In Section \ref{sec:mathematical_models}, we describe the mathematical models used in our numerical investigation: the (nonlinear) QGE and two of its simplifications - the linear Stommel model and the linear Stommel-Munk model.
Finally, in Section \ref{sec:Tests} we present a careful numerical investigation of the FE discretization of the streamfunction formulation of the QGE \eqref{eqn:FEForm} with the Argyris element.
The numerical results are benchmarked against those in the published literature.
The rates of convergence of the FE discretization are compared to the theoretical rates in Theorem \ref{thm:EnergyNorm} and Theorem \ref{thm:Errors}.


==> rate.tex <==
%\subsubsection{Method} \label{sss:Method}
Initially for each numerical test a uniform mesh size of $h=\frac{1}{2}$ is created, and then the mesh
is refined by halving the size of the triangle. The refined results correspond to a mesh size of $h=\frac{1}{4}$.  This
process of mesh refinement is repeated a total of four times resulting in numerical solutions for mesh sizes
corresponding to $h=\left\{\frac{1}{2},\frac{1}{4},\frac{1}{8},\frac{1}{16},\frac{1}{32}\right\}$. 
%\input{Mesh.tex}

After the FE code is run for each $h$, the corresponding $\psi^h$ is used to calculate the errors $e_0,\, e_1,\text{
and } e_2$, where $e_0,\, e_1,\text{ and } e_2$ are the $L^2,\, H^1,$ and $H^2$ errors respectively, and are
given by 
%{\small
\begin{align*}
  e_0 &= \left(\int_{\Omega}\!\left( \psi^h - \psi \right)^2 \,d\vec{x}\right)^{\nicefrac{1}{2}}\\
  e_1 &= \left(e_0^2 + \int_{\Omega}\!  \left( \psi^h_x - \psi_x \right)^2 + \left( \psi^h_y - \psi_y \right)^2
    \,d\vec{x}\right)^{\nicefrac{1}{2}}\\
  e_2 &= \left(e_1^2 + \int_{\Omega}\!  \left( \psi^h_{xx} - \psi_{xx} \right)^2 + \left( \psi^h_{xy} - \psi_{xy}
    \right)^2 + \left( \psi^h_{yy} - \psi_{yy} \right)^2 \,d\vec{x}\right)^{\nicefrac{1}{2}}\\
\end{align*}
%}
The order of convergence, $O$, is then determined by calculating 
\begin{equation*}
  O = \dfrac{\log e_{\alpha}^i - \log e_{\alpha}^{i-1}}{\log h_i - \log h_{i-1}},
\end{equation*}
where $e_{\alpha}^i$ is the i$^{th}$ $\alpha$-error corresponding to the i$^{th}$ mesh size, $h_i$. 

Additionally, in each of the convergence data tables we also present the number of degrees of freedom (DoFs) for Argyris
Finite Elements. For the uniform mesh as described above and a rectangular domain of length, $L$, and height, $H$, the
DoFs are given by
\begin{equation*}
  %DoF = 6\cdot\left(\frac{L}{h}+1\right)\cdot\left(\frac{H}{h}+1\right)+\frac{L}{h}\cdot\left(\frac{H}{h}+1\right)+\left(2\frac{L}{h}+1\right)\cdot\frac{H}{h}.
  N = \frac{7h\left(H + L\right) + 9 H L}{h^2} + 6.
\end{equation*}

